AequeVox: Automated Fairness Testing of Speech Recognition Systems

Automatic Speech Recognition (ASR) systems have become ubiquitous. They can be found in a variety of form factors and are increasingly important in our daily lives. As such, ensuring that these systems are equitable to different subgroups of the population is crucial. In this paper, we introduce, AequeVox, an automated testing framework for evaluating the fairness of ASR systems. AequeVox simulates different environments to assess the effectiveness of ASR systems for different populations. In addition, we investigate whether the chosen simulations are comprehensible to humans. We further propose a fault localization technique capable of identifying words that are not robust to these varying environments. Both components of AequeVox are able to operate in the absence of ground truth data. We evaluated AequeVox on speech from four different datasets using three different commercial ASRs. Our experiments reveal that non-native English, female and Nigerian English speakers generate 109%, 528.5% and 156.9% more errors, on average than native English, male and UK Midlands speakers, respectively. Our user study also reveals that 82.9% of the simulations (employed through speech transformations) had a comprehensibility rating above seven (out of ten), with the lowest rating being 6.78. This further validates the fairness violations discovered by AequeVox. Finally, we show that the non-robust words, as predicted by the fault localization technique embodied in AequeVox, show 223.8% more errors than the predicted robust words across all ASRs.

==> Citations.tex <==
\section{Citations}
The use of \BibTeX\ for the preparation and formatting of one's
references is strongly recommended. Authors' names should be complete
--- use full first names (``Donald E. Knuth'') not initials
(``D. E. Knuth'') --- and the salient identifying features of a
reference should be included: title, year, volume, number, pages,
article DOI, etc.

==> FASE 2021/Citations.tex <==
\section{Citations}
The use of \BibTeX\ for the preparation and formatting of one's
references is strongly recommended. Authors' names should be complete
--- use full first names (``Donald E. Knuth'') not initials
(``D. E. Knuth'') --- and the salient identifying features of a
reference should be included: title, year, volume, number, pages,
article DOI, etc.

==> FASE 2021/Methodology-UserStudy.tex <==
\smallskip \noindent
\textbf{User Study:}
\label{sec:user-study-process}
In the course of our study, we subject speech signals to various metamorphic transformations (as explained in the preceding section) to test the overall robustness of ASR systems to these transformations. However, considering the full range of metamorphic transformations \revise{may} not useful since certain transformations deform speech to such an extent that it \revise{may not} be recognised any longer. In order to identify the set of transformations that are meaningful to consider, we conducted a study on relative comprehensibility of the transformed speech. The user study sought to determine whether the metamorphic transformations applied to the speech resulted in a speech that was still comprehensible to humans. Specifically, we seek to identify the degree to which the speech remains comprehensible as the intensity of each transformation is increased.


\textbf{User Study Setup:} We conducted a user study using Amazon’s mTurk platform. In particular, 200 participants were presented with an audio file containing speech utterances by a {\em female native English speaker}. In addition, the audio clip contained nearly all the sounds in the English language to represent the full spectrum of the language, as found in Speech Accent Archive~\cite{accents}. Users were presented with the original audio file along with a set of transformed speech files in order of increasing intensity. For instance, in the case of the "Scale" transformation, participants were first presented with a file that was slightly slowed down and subsequent files were slowed down even further. Users then rated the comprehensibility of the speech files in comparison to the original audio file. The rating was on a 1 to 10 scale, where "10" refers to the case where the modified speech file was just as comprehensible as the original speech and "1" refers to the case where 
the modified speech was not comprehensible at all.  

Participants were required to rate the comprehensibility of the entire set of transformations under 
study i.e. Amplitude, Clipping, Drop, Frame, Highpass, Lowpass, Noise and Scale 
(see~\Cref{fig:soundwave-transform}). The average score of each transformation was used to determine 
the comprehensibility score. In general, we see that 
the comprehensibility of the speech tends to go down as the intensity of the transformation increases, 
as observed in~\Cref{fig:user-study-results}. We present a comprehensive analysis of the user study results in {\bf RQ2}. 

%\smallskip \noindent
%\textbf{Caveats:} In conducting the study, two assumptions were made. Firstly, we assume that the degree to which comprehensibility changes when subject to transformations is independent of the characteristics of the speaker’s voice. Secondly, we assume that the speech is reflective of the broader English language. That is we assume that the comprehensibility of speech when subject to transformations is independent of the words contained in it. In the fullness of time, a larger scale user study could be performed to verify the results.

%\todo{Check: Caveats section is possibly superfluous. Possibly moved to threats to validity.}


==> FASE 2021/abstract.tex <==
\begin{abstract}
Automatic Speech Recognition (ASR) systems have become ubiquitous. They can be found in a variety of form factors and are increasingly important in our daily lives. As such, ensuring that these systems are equitable to different subgroups of the population is crucial.
%
In this paper, we introduce, \SMLT, an automated testing framework for evaluating the fairness of ASR systems. \revise{\SMLT simulates different environments to assess the effectiveness of ASR systems for different populations. In addition, we investigate whether the chosen simulations are comprehensible to humans. We further propose a fault localization technique capable of identifying words that are not robust to these varying environments.} Both components of \SMLT are able to operate in the absence of ground truth data.

We evaluated \SMLT on speech from four different datasets using three different commercial ASRs. Our experiments reveal that non-native English, female and Nigerian English speakers generate
{\em 109\%}, {\em 528.5\%} and {\em 156.9\%} more errors, on average than
native English, male and UK Midlands speakers, respectively. 
%
%\revise{
Our user study also reveals that 82.9\% of the simulations (employed through speech transformations) had a 
comprehensibility rating above seven (out of ten), with the lowest rating being 6.78. This further validates 
the fairness violations discovered by \SMLT. Finally, we show that the non-robust words, as predicted 
by the fault localization technique embodied in \SMLT, show {\em 223.8\%} more errors than the predicted 
robust words across all ASRs.
%}.

%The user study reveals that {\em 82.9\%} of the metamorphic transformations had a comprehensibility rating above 7. Additionally, we show that the predicted non-robust words show {\em 223.8\%} more errors than the predicted robust words across all ASRs and that non-Native English speakers show {\em 29.8\%} more faults
%in comparison to native English speakers.
 
\end{abstract}


==> FASE 2021/background.tex <==
\section{Background}
\label{sec:background}

In this section, we introduce the necessary background information. 

%\smallskip \noindent
%\textbf{ASR Systems:} Automatic Speech Recognition (ASR) is now ubiquitous and found in all facets of life. Smart home devices with digital assistants utilize ASR to parse commands and questions. Today's mobile phones also come equipped with digital assistants (e.g. Google Assistant and Siri) capable of understanding and responding to voice queries. ASR systems also power voice typing applications seen on phones. Such functionality is also increasingly making its way onto our desktop operating systems (e.g. Siri on MacOS and Cortana on Windows).
%
%This explosion in use has positive implications for both the accessibility and availability of technology. For instance, individuals that struggle with using the phone due to temporary or permanent disabilities can make use of these technologies to accomplish tasks more easily. Illiterate individuals, on the other hand, could better communicate with aid of these systems. This makes it particularly important to ensure that these systems are fair to individuals belonging to a variety of groups.

\smallskip \noindent
\textbf{Fairness in ASR Systems:}
%Some researchers have drawn attention to the unfair nature of ASR systems. 
%One such work is 
\revise{A recent work, FairSpeech~\cite{racialASR}, 
%It examines the gap in 
%effectiveness of ASR systems between white speakers and black speakers. 
uses conversational speech from black and white speakers 
%to test different ASR systems 
to find that the word error rate for individuals who speak 
African American Vernacular English (AAVE) is nearly twice as large in all 
cases.}
%even accounting for differences in transcription quality.

%\smallskip \noindent
%\textbf{Fairness Testing:}
%Assessing the fairness of systems in an automatic manner is an active area of 
%research and many papers propose to test such systems. Themis~\cite{themis} 
%proposes formal definitions for algorithmic fairness and introduces a technique 
%to measure discrimination in software. Aequitas~\cite{aequitas} seeks to generate 
%test inputs that violate fairness through probabilistic search of the input space.

\smallskip \noindent
\textbf{Testing ASR Systems:}
The \revise{major} testing focus, till date has been on image recognition systems and large language 
models. Few papers have probed ASR systems. One such work, Deep-Cruiser~\cite{deepcruiser} applies metamorphic transformations 
to audio samples to perform coverage-guided testing on ASR systems. 
Iwama et al.~\cite{automatedBasicRecognition} also perform automated testing on the basic recognition capabilities of ASR systems to detect functional defects.
%in early stages of development of ASR systems. 
CrossASR~\cite{crossASR} is another recent paper that applies differential testing 
to ASR systems. 
%It obviates the need for manually labeled data by employing Text to Speech (TTS) 
%engines to synthesize inputs that are then fed to different ASR systems to find erroneous 
%transcriptions.

\smallskip \noindent
\textbf{The Gap in Testing ASR Systems:}
There is little work on automated methods to formalise and test fairness in ASR systems. 
In this work, we present \SMLT to test the fairness of ASR systems 
with respect to different population groups. It accomplishes this with the aid of differential testing 
of speech samples that have gone through metamorphic transformations of varying intensity. 
%Given speech from different groups of speakers, \SMLT applies a variety of meaningful 
%transformations to the speech. The transformed speech is then fed to two different ASR systems. 
%The results from these systems are compared and a distance metric is generated for each 
%individual transformation. We then compute the change in this distance metric between the 
%original and transformed speech. Finally, we compare the degree to which the metric changes for each group.
\revise{Our experimentation suggests that speech from different \revise{groups} of speakers receives significantly different quality of service across ASR systems.}
%We also find that speech from native English speakers 
%tends to be more robust to transformations than speech from speakers from other population groups. 
In the subsequent sections, we describe the design and evaluation of our \SMLT system. 



==> FASE 2021/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this work we introduce \SMLT, an automated fairness testing 
technique for ASR systems. To the best of our knowledge, 
we are the first work that explores considerations beyond error
rates for discovering fairness violations. We also show that the 
speech transformations used by \SMLT are largely comprehensible
through a user study. 
Additionally, \SMLT highlights words where a given ASR system exhibits
faults, and we show the validity of these explanations. These faults 
can also be used to identify unfairness in ASR systems. 
%Subsequently, cases where \SMLT is not applicable are identified. 

\SMLT is evaluated on three ASR systems and we use four distinct datasets. 
Our experiments reveal that speech from non-native English, female and Nigerian 
English speakers exhibit more errors, on average than speech from native English, 
male and UK Midlands speakers, respectively. We also validate the fault 
localization embodied in \SMLT by showing that the predicted non-robust 
words exhibit {\em 223.8\%} more errors than the predicted robust words 
across all ASRs.

%{\em 109\%}, {\em 528.5\%} and {\em 156.9\%} more errors, on average than 
%native English, male and UK Midlands speakers, respectively. The user study 
%reveals that {\em 82.9\%} of the metamorphic transformations 
%had a comprehensibility rating above seven (out of ten).
%Additionally, we show that the predicted non-robust words show 
%{\em 223.8\%} more errors than the predicted robust words across all ASRs 
%and that non-Native English speakers show {\em 29.8\%} more faults 
%in comparison to native English speakers. 
%\todo{Please add appropriate summary for rq5}

We hope that \SMLT drives further work on systematic fairness testing of 
ASR systems. To aid future work, we make all our code and data publicly 
available: \textbf{https://github.com/sparkssss/AequeVox}
%\begin{center}
%        
%\end{center}
 

==> FASE 2021/datasets.tex <==
\section{Datasets and Experimental Setup}
\label{sec:experimental-setup}
%In this section, we discuss the experimental settings used for the evaluation 
%of \SMLT. 

\smallskip \noindent
\textbf{ASR Systems under Test:}
We evaluate \SMLT on three commercial ASR systems from Google Cloud Platform (GCP), IBM Cloud, and Microsoft Azure. 
\revise{We use the standard models for GCP and Azure, and the {\em BroadbandModel} for IBM. }
%For GCP, we evaluate speech samples using the standard model with the language set to ‘en-us’. For IBM Cloud, we use the ‘en-US\_BroadbandModel’ with no additional parameters. Finally, we use Azure’s standard model with the language set to ‘en-us’.
In all three cases, the audio samples were identically encoded as .wav files using Linear 16 encoding.

%\smallskip \noindent
%\textbf{Speech Transformations: }
%In the experiments conducted, we leverage eight different types of simple transformations: noise addition, amplitude scaling, amplitude clipping, drop, frame, high pass filters, low pass filters and frequency scaling. 
\revise{In each of the following transformations, we vary a parameter, $\theta$. We call this the transformation parameter.}
\revise {
Some of the transformations have abbreviations within parentheses. 
Such abbreviations are used in later sections to refer to the respective transformations.}

%\revise{}
\smallskip \noindent
\textbf{Amplitude Scaling (Amp)}: For amplitude scaling, we scale 
the audio sequence by a constant by multiplying
each individual audio sample by $\theta$.
%\textbf{Amplitude Scaling and Clipping:} For the case of amplitude scaling, we scale 
%the input audio sequence by a constant factor $\theta$. More specifically, we multiply 
%each individual audio sample by $\theta$.
%
%\textbf{Amplitude Clipping:}

%\revise {}
\smallskip \noindent
\textbf{Clipping:} \revise{The audio samples are scaled such that their 
amplitude values are bound by [$-1$, $1$]. \SMLT then clips these samples such that the amplitude range is [$-\theta$, $\theta$]. 
These clipped samples are then rescaled and encoded.}

%For clipping, we use $\theta$ to specify the upper and lower bounds for the amplitude of the audio signal. 
%%We set any individual audio sample with a value higher or lower than the upper and lower 
%%bounds respectively to be equivalent to the bounding values. 
%We scale the original audio such that the value that 
%can be taken by an individual sample is 1 and -1 respectively. 
%We set $\theta$ and $-\theta$ to be the 
%upper bound and to be the lower bound for the amplitude. 
%We then 
%rescale the audio files 
%appropriately to make it more conducive for encoding as a Linear 
%16 wave file. 

\smallskip \noindent
\textbf{Drop/Frame:} \revise{For Drop, 
\SMLT divides the audio into 20ms chunks. 
$\theta$\% of these chunks are then randomly discarded (amplitude set 
to zero) from the audio. For Frame, \SMLT divides the audio into $
\theta$ms chunks and 10\% of these chunks are then randomly discarded. No two adjacent chunks are discarded.}
%First, we divide the audio file into chunks of 20ms. We then randomly choose 
%chunks and set all the individual samples within the time window to be 0 taking care to ensure 
%that no two adjacent chunks are chosen. Here, we use $\theta$ to determine the percentage 
%of audio that is cut off in this manner. For instance, for a $\theta$ value of 10, we  
%ensure that 10\% of the entire audio file is set to zero.

%\smallskip \noindent
%\textbf{Frame:} \revise{\SMLT divides the audio into $\theta$ms chunks.
%10\% of these chunks are then randomly discarded from the audio 
%(amplitude set to zero). No two adjacent chunks are discarded}

%We repeat the procedure used for Drop, while keeping the percentage of the 
%audio that is cut off at a constant 10\%. Instead, we subdivide the files into $\theta$ms 
%long chunks. For instance, for a $\theta$ value of 10, we would subdivide the audio file 
%into 10ms chunks and replace all the samples within the chosen chunks with 0s. We also 
%ensure that the total percentage of audio eliminated in this manner remains at a constant 
%10\%.

%\smallskip \noindent
%\textbf{High Pass Filter:}

%\revise {}
\smallskip \noindent
\textbf{High Pass (HP)/ Low Pass (LP) Filter:} 
\revise{Here we apply a butterworth~\cite{butterworth} filter of order two to the entire audio file with $\theta$ determining the cut-off frequency.}
%For instance, 
%for a $\theta$ value of 600, we would apply a second order butterworth filter with a cutoff frequency of 600 Hz to the entire signal.

%\smallskip \noindent
%\textbf{Low Pass Filter:}

%\revise {}
%\smallskip \noindent
%\textbf{Low Pass Filter (LP):} Similarly, we apply a second order low pass butterworth filter 
%with a cutoff frequency of $\theta$ to achieve this transformation.

%\smallskip \noindent
%\textbf{Noise Addition:}

%\revise {}
\smallskip \noindent
\textbf{Noise Addition (Noise):} \revise{
$\theta$ represents signal to noise 
(SNR) ratio~\cite{snr-def} of the transformed audio signal. 
A lower $\theta$ means higher noise in the transformed audio.}

%First, we compute the root mean squared value of the entire audio 
%signal. We then use $RMS\textsubscript{Noise}=\sqrt{\frac{RMS_{Signal}^{2}}{10^{\frac{\theta}{10}}}}$
%to compute the root mean squared value for the noise. We then sample from a Gaussian distribution with mean 0 and standard deviation equal to $RMS\textsubscript{Noise}$. The resultant array of noise samples is then added to the original signal.

%\smallskip \noindent
%\textbf{Frequency Scaling:}

%\revise {}
\smallskip \noindent
\textbf{Frequency Scaling (Scale):} \revise{In this case, 
$\theta$ is the sampling frequency. The lower the value of $\theta$, the slower the audio. 
In this transformation, the audio is slowed down 
$\theta$ times.}

% Lastly, we have frequency scaling, where we vary the sampling com
%frequency of the audio file by $\theta$. For instance, for a $\theta$ value of 0.8, we 
%slow down the entire audio file by sampling it at a rate 0.8 times the original sampling rate.

\revise{\Cref{tab:transList} lists all the different values used for 
$\theta$. An additional parameter ($\theta = 2.0$) is used for 
{\em Amp}.}

\begin{table}[t]
\caption{Transformations Used}
\centering
	{\scriptsize
    \begin{tabular}{l p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}p{1cm}}
        \toprule
        \multicolumn{1}{l}{Transformation Type}  & \multicolumn{5}{c}{$\theta$ Used}  \\ \midrule
        \multicolumn{1}{l}{}  & \multicolumn{5}{c}{Least Destructive $\longrightarrow$ Most Destructive} \\  \cmidrule{2-6}
        Amplitude & 0.5 & 0.4 & 0.3 & 0.2 & 0.1 \\
        Clipping & 0.05 & 0.04 & 0.03 & 0.02 & 0.01 \\
        Drop & 5 & 10 & 15 & 20 & 25 \\
		Frame & 10 & 20 & 30 & 40 & 50 \\
		HP & 500 & 600 & 700 & 800 & 900 \\
		LP & 900 & 800 & 700 & 600 & 500 \\
		Noise & 10 & 8 & 6 & 4 & 2 \\
		Scale & 0.9 & 0.8 & 0.7 & 0.6 & 0.5 \\
		\bottomrule


    \end{tabular}}
    \label{tab:transList}
\end{table}

\begin{table}[t]
\caption{Datasets Used}
\centering
	{\scriptsize
	%\begin{tabular}{@{}llllll@{}}
    \begin{tabular}{l r rrr}
        \toprule 
        Dataset & \makecell{Duration(s)} & \#Clips & \makecell{\#Distinct\\Speakers} 
         \\ \midrule
        Accents  & 25-35 & 28 & 28  \\
%        \begin{tabular}[c]{@{}l@{}}Native English speakers,\\ native French speakers,\\ native Ganda speakers,\\ native Indonesian speakers,\\ native Korean speakers,\\ native Russian speakers\end{tabular} \\
        RAVDESS  & 3 & 32 & 8  \\
%        \begin{tabular}[c]{@{}l@{}}Male speakers,\\ female speakers\end{tabular} \\
		Midlands  & 3-5 & 4 & 4 \\
%		Midlands english speakers \\
		Nigerian English & 4-6 & 4 & 4 \\
%		& Nigerian english speakers \\
		\bottomrule
    \end{tabular}}
    \label{tab:dataList}
\end{table}


\smallskip \noindent
\textbf{Datasets: }
\revise{We use the Speech Accent 
Archive (Accents)~\cite{accents}, the Ryerson Audio-Visual Database of Emotional Speech and Song (RAVDESS)~\cite{ravdess}, Multi speaker Corpora of the English Accents in the British Isles (Midlands)~\cite{uk-midlands-dataset}, and a Nigerian English speech dataset~\cite{nigerian-english} to evaluate \SMLT taking care to ensure male and female speakers are equally represented. \Cref{tab:dataList} provides additional details about the setup.}

%\revise{
%\smallskip \noindent
%\textbf{Speech Accent Archive:} We examine seven different groups of speakers from this dataset,
%namely, native English speakers, native French speakers, native Ganda speakers, native Gujarati
%speakers, native Indonesian speakers, native Korean speakers, and native Russian speakers. For 
%each individual group, we select speech samples from two female and two male speakers. When more
%speech samples exist in the dataset, we randomly choose from the available samples. Concretely,
%we obtain a total of four sets of approximately 25 to 35 seconds long speech samples for each group
%under test.%}

%\revise{
%\smallskip \noindent
%\textbf{CORAAL:} We examine one group of speakers from this dataset, namely, speakers that speak
%African American Vernacular English (AAVE). From this dataset, we randomly choose two female
%and two male speakers. Since the dataset itself consists of long form interviews,
%we cut out audio samples of approximately 5 seconds in length for use in our experimentation.
%Concretely, we obtain a total of 4 sets of speech samples that are approximately 5 seconds long
%for the group under test.%}

%\revise{
%\smallskip \noindent
%\textbf{RAVDESS:} We examine two groups of speakers from this dataset, namely female and male
%speakers. For each group, we randomly select 4 speakers. We then obtain four sets of speech
%samples from each individual with two sets consisting of the individual speaking 
%utterance one and the other two sets consisting of the individual speaking 
%utterance two. Concretely, we obtain 16 sets of speech samples that are approximately 3 seconds
%long for each group under test.%}

%\revise{
%\smallskip \noindent
%\textbf{Midlands:} We examine one group of speakers from this dataset, namely, speakers speaking
%the Midlands English dialect of speech. From this dataset, we randomly choose two female 
%Midlands English speakers and two male Midlands English speakers. We then obtain a speech sample
%from each individual. Concretely, we obtain 4 sets of speech samples that are approximately
%3 to 5 seconds long for the group under test.%}

%\revise{
%\smallskip \noindent
%\textbf{Nigerian English:} We examine one group of speakers from this dataset, namely, Nigerian
%English speakers. We randomly choose two female and two male speakers from this dataset. We then
%obtain a speech sample from each individual. Concretely, we obtain 4 sets of speech samples
%that are approximately 4 to 6 seconds long for the group under test.%}


%In the case of the Speech Accent Archive, we select 
%speech samples from two female and two male speakers for each accent tested. When multiple speech 
%samples exist, we choose randomly from the available samples. For CORAL, we select speech from two 
%randomly chosen male and two randomly chosen female speakers and generate the test files by 
%cutting audio of approximately five seconds long from the interviews.  Similarly, we randomly select 
%four male and four female speakers from the RAVDESS dataset. We then obtain four sets of speech 
%samples from each individual with two sets consisting of the individuals speaking utterance one and 
%the other two sets consisting of the individuals speaking utterance two. For the Midlands dataset, 
%we similarly choose four sets of speech samples from individuals residing in the Midlands taking 
%into account two different female and two different male speakers. Lastly, for the Nigerian English 
%dataset, we choose speech samples from two different females and two different males.

%\subsection{Comparison Setup}
%Actual Thresholds


==> FASE 2021/introduction.tex <==
\section{Introduction}



%\todo{Sudipta please see Formalising Fairness in ASRs for formalising 
%unfairness. The definitions are seen in Section 3.1.1 and Section 3.2.7
%in \cite{fairnessDefinitions}}



Automated speech recognition (ASR) systems have made great 
strides in a variety of application areas e.g. smart home devices, robotics 
and handheld devices, among others.
\revise{
The wide variety of applications have made ASR systems serve 
increasingly diverse groups of people.
}
%Considering the potential application areas 
%offered by ASR systems, ASR systems are now available to a diverse group 
%of people. 
Consequently, it is crucial that such systems behave in 
a non-discriminatory fashion. 
%that are not discriminatory in nature.
%
This is particularly important because assistive technologies powered by 
ASR systems are often the primary mode of interaction 
for users with certain disabilities~\cite{assistiveSpeech}.
% 
%For example, consider a voice assistant system as a tool for 
%communication. This is often the primary
%mode of interaction with technology for people with certain disabilities.
Consequently, it is 
critical that an ASR system employed in such systems is effective in 
diverse environments and across a wide variety of speakers 
(e.g. male, female, native English speakers, non-native English speakers)
\revise{since they are often deployed in safety-critical 
scenarios~\cite{goss2016incidence}.}

In this paper, we are broadly concerned with the {\em fairness properties 
in ASR systems}. Specifically, {\em we investigate whether speech 
from one group is more robustly recognised as compared to another group}. 
For instance, consider the example shown in \Cref{fig:intro-diagram} for 
a system $\mathit{ASR}$. The metric $\mathit{ASR}_{\mathit{Err}}$ captures 
the error rate induced by $\mathit{ASR}$. Consider speech from two 
groups of speakers i.e. {\em male} and {\em female}. We assume that the 
$\mathit{ASR}$ has similar error rates for both the groups of speakers, 
as illustrated in the upper half of \Cref{fig:intro-diagram}. We now apply 
a small, constant perturbation on the speech provided by the two groups. 
Such a perturbation can be, for instance, addition of small noise, 
exemplifying the natural conditions that the ASR systems may need to work 
in (e.g. a noisy environment). If we observe that the $\mathit{ASR}_{\mathit{Err}}$ 
increases disproportionately for one of the speaker groups, as compared to 
the other, then we consider such a behaviour a violation of fairness (see 
the second half of \Cref{fig:intro-diagram}). 
\revise{Intuitively, \Cref{fig:intro-diagram} exemplifies the violations 
of {\em Equality of Outcomes}~\cite{phillips2004defending} in the context of ASR systems, 
where the male group is provided with a higher quality of service in a noisy 
environment as compared to the female group. Automatically discovering such 
scenarios of unfairness via simulating the ASR service in diverse 
environment is the main contribution of our \SMLT framework. }


%In short, we formalize 
%the notion of fairness and discover the group fairness violations in ASR
%systems~\cite{fairnessDefinitions}. 


\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.1]{figs/intro-diagram.png}
\end{center}
\vspace{-0.2in}
\caption{Fairness Testing in \SMLT}
\label{fig:intro-diagram}
\vspace{-0.2in}
\end{figure}

%
%Given speech from different groups of people (e.g. male and female), it is 
%possible to explore different perturbations of the speech and check the 
%behaviour of ASR systems against such perturbations. In this paper, we 
%conceptualize, design and evaluate \SMLT \footnote{From the Latin for equal 
%({\em aeque}) and voice ({\em vox})}, a differential testing methodology 
%to automatically discover fairness violations in ASR systems. Moreover, 
%\SMLT employs a systematic fault localization method, which, in turn highlights
%the words contributing to errors in ASR. To the best of our knowledge, 
%{\em \SMLT is the first fairness testing methodology to automatically discover and 
%localize errors in ASR systems.}

%To facilitate fairness testing of ASR systems, we face two main challenges. 

\SMLT facilitates fairness testing without having any access to ground truth 
transcription data. 
%Firstly, for the fairness testing of speech, we should have access to 
%large samples of manually transcribed speech. 
Although, text-to-speech (TTS) can be used for generating speech, we argue that 
it is not suitable for accurately identifying the bias towards speech coming from 
a certain group.
%
%\revise{
Specifically, speakers may intentionally use enunciation, 
intonation, different degrees of loudness or other aspects of vocalization 
to articulate their message. Additionally, speakers unintentionally 
communicate their social characteristics such as their place of origin 
(through their accent), gender, age and education. This is unique 
to human speech and TTS systems cannot faithfully capture all the complexities 
inherent to human speech. %}
% 
%Specifically, in speaking, speakers may intentionally introduce certain acts 
%such as persuading and directing. Moreover, speakers can use enunciation, 
%intonation or different degrees of loudness or other aspects of vocalization 
%to articulate the message. 
%
Therefore, we believe that fairness testing of ASR 
systems should involve speech data from human speakers. 

We note that human speech (and the ASRs) may be subject to adverse environments (e.g. 
noise) and it is critical that the fairness evaluation considers such 
adverse environments. 
\revise{To facilitate the testing of ASR systems in adverse 
environments, we model the speech signal %we derive meaningful metamorphic transformations for speech by 
as a sinusoidal wave 
and subject it to eight different 
metamorphic transformations (e.g. noise, drop, low/high pass filter) that 
are highly relevant in real life.} Furthermore, in the absence of manually 
transcribed speech, we use a differential testing methodology to expose 
fairness violations.
In particular, \SMLT identifies the bias in ASR systems via a two step approach: 
Firstly, \SMLT registers the increase in error rates for speech from two groups 
when subjected to a metamorphic transformation. Subsequently, if the increase 
in the error rate of one group exceeds the other by a given threshold, \SMLT 
classifies this as a violation of fairness. 
%
To the best of our knowledge, we are unaware of any such differential testing 
methodology. \revise{As a by product of our \SMLT framework, we highlight words 
that contribute to errors by comparing the word counts from the original speech. 
This information can be further used to improve the ASR system.}

%
%In particular, 
%we quantify the bias of ASR systems by observing the uneven increase in differential 
%testing error for one group in comparison to another (for a given transformation). 
%
%In our experiments, we observe that for a given transformation 
%has higher 
%
%towards a group via the difference between 
%the outputs of two ASRs. Consequently, we model fairness violations when the  
%bias scores computed for different groups differ beyond a certain threshold. 


%Furthermore, to facilitate the testing of ASR systems in adverse 
%environment, we derive meaningful metamorphic transformations for speech by 
%modeling it as a sinusoidal wave. 

%we combine concepts of Electrical Engineering and software testing, 
%specifically, to model the transformation of speech wave as metamorphic 
%transformations and subject these transformed speech signal for differential 
%testing. 

%\SMLT systematically combines metamorphic transformation and differential 
%testing. In particular, we subject the speech signal to eight different 
%metamorphic transformations (e.g. noise, drop, low/high pass filter) that 
%are highly relevant in real life. While applying these transformations, 
%the aim of \SMLT is to check whether the speech from certain groups 
%(e.g. female speakers) induces more errors in the ASR systems 
%as compared to the speech from other groups (e.g. male speakers). 
%Moreover, \SMLT can also be used to highlight words that contribute 
%to errors by comparing the word counts from the original speech. 
%This information can be further used to improve the ASR system.


\revise{Existing works~\cite{themis,aequitas} isolate certain sensitive 
attributes (e.g. gender) and use such attributes to test for fairness. 
%This is challenging to do in speech data. 
Isolating these attributes is
difficult in speech data, making it challenging to apply existing techniques to evaluate 
the fairness of ASR systems. \SMLT tackles this by
formalizing a unique fairness criteria targeted at ASR systems.}
%
%To fill this gap in fairness testing 
%for ASR systems, \SMLT formalizes a unique fairness criteria targeted at ASR systems.}
%\SMLT targets fairness in ASR systems. ASR systems are unique in the sense 
%that, unlike previous works in fairness testing, the input to ASR systems 
%are continuous signals. Thus, the generic fairness testing 
%methodologies are not applicable for fairness testing of ASR systems. 
Despite some existing efforts in testing ASR systems~\cite{crossASR,deepcruiser}, 
these  are not directly applicable for fairness testing. Additionally, some of these 
works require manually labelled speech transcription data~\cite{deepcruiser}. 
Finally, differential testing via TTS~\cite{crossASR} is not appropriate 
to determine the bias towards certain speakers, as they might use different 
vocalization that might be impossible (and perhaps irrational) to generate 
via a TTS. In contrast, \SMLT works on speech signals directly and defines 
transformations directly on these signals. \SMLT also does 
not require any access to manually labelled speech data for discovering 
fairness violations. 
%
%The remainder of the paper is organized as follows. After providing a brief 
%background (\Cref{sec:background}), we make the following contributions: 
%
In summary, we make the following contributions in the paper: 
\begin{enumerate}
%\item \revise{We formalize a notion of fairness and postulate
%that this fairness criteria should factor into the assessment of 
%state-of-the-art ASR systems. Incorporating this ensures that Equality of 
%Outcomes~\cite{phillips2004defending} in ASR systems is preserved  
%in different environments.}
%\todo{Sakshi personally prefers the previous version because QoS is standard term and aids clarity.}
%
%
%\item \revise{We formalize a notion of fairness in the quality of service 
%(QoS) provided by state-of-the-art ASR systems. Our formalization draws 
%connection with the Equality of Outcomes~\cite{phillips2004defending} in 
%the QoS provided by ASR systems in different environments.}
%propose a methodology 
%\SMLT, which leverages differential testing to uncover group fairness 
%violation in ASR systems (\Cref{sec:methodology}). 

\item \revise{We formalize a notion of fairness for ASR systems. This 
formalization draws parallels between the Equality of
Outcomes~\cite{phillips2004defending} and the quality of service provided 
by ASR systems in varying environments. }

\item \revise{We present \SMLT, which systematically combines 
metamorphic transformations and differential testing to highlight whether 
speech from a certain group (e.g. female) is subject to fairness violations 
by ASR systems. \SMLT neither requires access to ground truth transcription 
data nor does it require access to the ASR model structures}. 

%\item We conduct a user study with 200 users in Amazon mTurk to show that 
%the transformed speech signal used in our testing had high comprehensibility 
%(\Cref{sec:methodology}). 

\item We propose a fault localization method to identify the different words 
contributing to fairness errors.% (\Cref{sec:methodology}). 

%\item We provide an implementation of \SMLT and discuss its experimental 
%settings in detail to aid in replication (\Cref{sec:experimental-setup}). 

\item We evaluate \SMLT with three different ASR systems namely Google Cloud, 
Microsoft Azure and IBM Watson. We use speech from the 
Speech Accent Archive~\cite{accents}, 
%the Corpus of Regional African American Language (CORAAL)~\cite{aave}, 
the Ryerson Audio-Visual Database of Emotional Speech and Song (RAVDESS)~\cite{ravdess}, 
Multi speaker Corpora of the English Accents in the British Isles 
(Midlands)~\cite{uk-midlands-dataset}, and a Nigerian English speech dataset~\cite{nigerian-english}. 
Our evaluation reveals that speech from non-native English speakers and female 
speakers \revise{exhibit higher fairness violations as compared 
to native English speakers and male speakers, respectively}. %(\Cref{sec:results}). 

\item We validate the fault localization of \SMLT by showing that the identified 
{\em faulty} words generally introduce more errors to ASR systems even 
when used within speech generated via TTS systems. The inputs to the TTS system 
are randomly generated sentences that conform to a valid grammar. %(\Cref{sec:results}). 

\item We evaluate (via the user study) the human comprehensibility score of the 
transformations employed by \SMLT on the speech signal. The lowest comprehensibility 
score was 6.78 and 82.9\% of the transformations had a comprehensibility score of more 
than seven. %(\Cref{sec:results}). 
\end{enumerate}

%After discussing the threats to validity (\Cref{sec:threats}), we conclude in \Cref{sec:conclusion}. 


 
























==> FASE 2021/methodology.tex <==
\section{Methodology}
\label{sec:methodology}
%\smallskip \noindent

In this section, we discuss \SMLT in detail. In particular, 
we motivate and formalize the notion of {\em fairness} in ASR systems. 
Then, we discuss our methodology to systematically find the violation of 
fairness in ASR systems. The notations used are described in 
\Cref{tab:Notation}.

\begin{table}[t]
\caption{Notations used}
\centering
\resizebox{\linewidth}{!}{
    \begin{tabular}{lp{14cm}}
        \toprule
        Notation & Description \\ \midrule
	    $GR_B$ & Base group  \\
	    $GR_k$ & $k \in (1, n)$. Various comparison group  \\
	    $MT$ & Metamorphic transformations \\
	    $ASR$ & Automatic Speech Recognition system under test \\
	    $\tau$ &  A user specified threshold beyond which the difference in 
	    word error rate for the base and comparison groups is considered 
	    a violation of individual fairness\\
        \bottomrule
    \end{tabular}}
    \label{tab:Notation}
\end{table}

\smallskip \noindent
\textbf{Motivation:} \revise{
Equality of outcomes~\cite{phillips2004defending} describes a state in which all people have approximately the same material wealth and income, or in which the general economic conditions of everyone's lives are alike. For a software system, equality of outcomes can be thought of as everyone getting the same quality of service from the software they are using. For a lot of software services, providing the same quality of service is baked into the system by design. For example, the results of a search engine only depend on the query. The quality of the result generally does not depend on any sensitive attributes such as race, age, gender and nationality. In the context of an ASR, the quality of service does depend on these sensitive attributes. This inferior quality of service may be especially detrimental in safety-critical settings such as emergency medicine~\cite{goss2016incidence} or air traffic management~\cite{kopald2013applying,helmke2016reducing}.}

\revise{
In our work, we show that the quality of service provided by ASR systems is vastly different depending on one’s gender/nationality/accent. Suppose there are two groups of people using an ASR system, males and females. They have approximately the same level of service when using this service at their homes. However, once they step into 
a different environment such as a noisy street, the quality of service drops notably for the female users, but 
does not drop noticeably for the male users. This is a violation of the principle of 
equality of outcomes (as seen for software systems) and more specifically, group 
fairness~\cite{dwork2012fairness}. Such a scenario is unfair (violation of group fairness) 
because some groups enjoy a higher quality of service than others.}

\revise{
In our work, we aim to automate the discovery of this unfairness. We do this by simulating the environment where 
the behaviour of ASR systems are likely to vary. The simulated environment is then enforced in speech from different groups. Finally, we measure how different groups are served in different environments.}


\smallskip \noindent
\textbf{Formalising Fairness in ASRs:}
In this section, we formalise the notion of fairness in the context of 
automated speech recognition systems (ASRs). The 
fairness definition in ASRs is as follows:
\begin{equation}
\begin{gathered}
	\left| \mathit{ASR}_{\mathit{Err}}(\mathit{GR}_{i}) - \mathit{ASR}_{\mathit{Err}}(\mathit{GR}_{j}) \right| \leq \tau 
	\label{eqn:simple-fairness}
\end{gathered}
\end{equation} 
Here, $\mathit{GR}_{i}$ and $\mathit{GR}_{j}$ capture speech from distinct groups 
of people. If the error rates induced by $\mathit{ASR}$ for group $\mathit{GR}_{i}$ 
($\mathit{ASR}_{\mathit{Err}}(\mathit{GR}_{i})$) and for group $\mathit{GR}_{j}$ 
($\mathit{ASR}_{\mathit{Err}}(\mathit{GR}_{j})$) differ beyond a certain threshold, 
we consider this scenario to be unfair. Such a notion of unfairness was studied in 
a recent work~\cite{racialASR}. 


In this work, we want to explore \revise{whether different groups are fairly treated under varying conditions.}
%the unfairness of two groups which have similar error rates with respect to an ASR.
%Specifically, we ask the following question: 
%{\em Are there considerations beyond error rates that we need to make?}
%Intuitively, we measure how robust speech from different groups of people is and 
%we check if certain groups fare better than the others. We characterise robustness 
%by transforming the speech and then checking whether such a transformation results 
%in a similar word error rate. 
\revise{Intuitively, we subject speech from different groups to a variety of 
simulated environments. We then measure the word error rates of the speech in such 
simulated environments and check if certain groups fare better than others. }
%\revise{By subjecting the speech to certain 
%transformation, we simulate the environment surrounding the speech (e.g. a noisy 
%street).}
%
%We characterise robustness 
%as a transformation of sound which changes it slightly. 
Formally, we capture the notion of fairness targeted by \SMLT as follows: 
\begin{equation}
\begin{gathered}
	D_{i} \gets  \mathit{ASR}_{\mathit{Err}}(\mathit{GR}_{i}) - 
	\mathit{ASR}_{\mathit{Err}}(\mathit{GR}_{i} + \delta)  \\
	D_{j} \gets  \mathit{ASR}_{\mathit{Err}}(\mathit{GR}_{j}) - 
	\mathit{ASR}_{\mathit{Err}}(\mathit{GR}_{j} + \delta) \\
	\left| D_{i} - D_{j}\right| \leq \tau 	
\label{eqn:robustness-fairness}
\end{gathered}
\end{equation} 
Here we perturb the speech of the two groups ($GR_{i}$ and $GR_{j}$) by 
adding some $\delta$ to the speech. We compare the degradation in the 
speech ($D_{i}$ and $D_{j}$). 
\revise{If the degradation faced by one group is far greater than the 
one faced by the other, we have a fairness violation. This is because  
speech from both groups ought to face similar degradation when subject 
to similar environments (simulated by $\delta$ perturbation) when 
equality of outcomes~\cite{phillips2004defending} holds. More 
specifically, this is a group fairness violation
because the quality of service (outcome) depends on 
the group~\cite{dwork2012fairness,fairnessDefinitions}.}

%If one group degrades much more than the 
%other, this is a group fairness violation~\cite{fairnessDefinitions}. 
%\revise{This is in line with our notion of fairness motivated by 
%the Equality of outcomes~\cite{phillips2004defending}. Specifically, 
%we expect the speech from groups $GR_{i}$ and $GR_{j}$ to face 
%similar degradation in terms of word error rates when the environment 
%is changed (simulated by $\delta$ perturbation) for both the groups.}

%speech from both groups $GR_{i}$ and $GR_{j}$ should have similar 
%error rates (bounded by threshold $\tau$) in an environment simulated 
%via perturbing the speech by $\delta$.}
%Specifically, this can be viewed as a violation of {\em group 
%fairness}~\cite{fairnessDefinitions}. If an utterance (perturbed 
%with the same $\delta$) is more likely to be recognised by an ASR
%for one group in comparison to another, then this is a violation of group 
%fairness.
%
%
%
%\smallskip \noindent
%\textbf{\SMLT fairness testing overview}
%
%%\todo{Add paragraph about not needing ground truth and using diff testing}




\begin{algorithm}[t]

	
    \caption{\SMLT Fairness Testing}
    {\scriptsize
    \begin{algorithmic}[1] 
        \Procedure{Fairness\_Testing}
        {$\mathit{GR}_B,\mathit{MT},\mathit{GR}_1, \cdots, \mathit{GR}_n,\tau, \mathit{ASR}_1, \mathit{ASR}_2$}
        	\State $Error\_Set \gets \emptyset$ 
        	
        	\For{$T \in \mathit{MT}$}
        	\State $\mathit{GR}_B^T \gets T(\mathit{GR}_B)$
        	\LineComment $\mathcal{L}$ computes the average 
        	word level levenshtein distance
        	\LineComment between the outputs of $\mathit{ASR}_1$ and $\mathit{ASR}_2$   
        	\State $d_B \gets \mathcal{L} (\mathit{ASR}_1(\mathit{GR}_B), \mathit{ASR}_2(\mathit{GR}_B))$
        	\State $d_B^T \gets \mathcal{L} (\mathit{ASR}_1(\mathit{GR}_B^T), \mathit{ASR}_2(\mathit{GR}_B^T))$
        	\State $D_B \gets d_B^T - d_B$

        		\For{$k \in (1, n)$}
        			\State $\mathit{GR}_k^T \gets T(\mathit{GR}_k)$
        			\State $d_k \gets \mathcal{L} ( \mathit{ASR}_1(\mathit{GR}_k), \mathit{ASR}_2(\mathit{GR}_k))$
        			\State $d_k^T \gets\mathcal{L} ( \mathit{ASR}_1(\mathit{GR}_k^T), \mathit{ASR}_2(\mathit{GR}_k^T))$
        			\State $D_k \gets d_k^T - d_k$
        			\If{$D_B - D_k > \tau$}
        				\State $Error\_Set \gets Error\_Set \cup 
        				(\mathit{GR}_B, \mathit{GR}_k, T)$
        			\EndIf
        		\EndFor
        	\EndFor
        	\State \Return $Error\_Set$
            
        \EndProcedure
    \end{algorithmic}
    }
    \label{alg:test-gen}
 \end{algorithm}





\smallskip \noindent
\textbf{Example:}
To motivate our system, let us sketch out an example. Consider texts of approximately 
the same length spoken by two sets of speakers whose native languages are 
$L_1$ and $L_2$ respectively. 
%a set of native language $L_1$ and another set of native native language $L_2$  
%speakers. 
Let us assume that both sets of speakers read out a text in English. \SMLT uses 
two ASR systems and obtains the transcript of this speech. \SMLT then employs 
differential testing to find the word-level levenshtein distance~\cite{levenshtein-dist} 
between these two sets of transcripts. 
Let us also assume that the \revise{average} 
word-level levenshtein distance is two and four for 
$L_1$ and $L_2$ native speakers, respectively. 

\revise{
\SMLT then simulates a noisy environment by adding noise to the speech and 
obtains the transcript of this transformed speech.}
%
%\SMLT then adds noise to the speech \revise{to simulate a noisy environment} 
%and obtains the transcript of this transformed speech as well. 
%
Let us assume now that the \revise{average} levenshtein distance
for this transformed speech is 4 and 25 for $L_1$ and $L_2$ native speakers, 
respectively. It is clear that the degradation for the speech of 
native $L_2$ speakers is much more severe. \revise{In this case, the quality of 
service that $L_2$ native speakers receive in noisy environments
is worse than $L_1$ native speakers. This is a violation of 
fairness which \SMLT aims to detect.} 

%\todo{discuss how to explain assumptions and why they hold}
The working principle behind \SMLT holds even if the spoken text is different. 
This is because \SMLT just measures the relative degradation in ASR performance 
for a set of speakers. For large datasets, we are able to measure the average 
degradation in ASR performance with respect to different groups of speakers 
(e.g. {\em male}, {\em female}, {\em native, non-native English} speakers). 
%\todo{I want to say that it does not matter what they are speaking the degradation is what should be captured. Also add points for speech not being equal length. Ask Sudipta}


\begin{figure*}[t]
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{cccc}
\includegraphics[scale=0.25]{figs/original.png} & 
\includegraphics[scale=0.25]{figs/uniform.png} & 
\includegraphics[scale=0.25]{figs/amplitude.png} & 
\includegraphics[scale=0.25]{figs/frequency.png}
 \\
{\bf (a)} & {\bf (b)} & {\bf (c)} & {\bf (d)}\\
\end{tabular}}
\\
\resizebox{\linewidth}{!}{
\begin{tabular}{cccc}
\includegraphics[scale=0.25]{figs/clipping.png} & 
\includegraphics[scale=0.25]{figs/dropframe.png} & 
\includegraphics[scale=0.25]{figs/lowpass.png} & 
\includegraphics[scale=0.25]{figs/highpass.png} \\
{\bf (e)} & {\bf (f)} & {\bf (g)} & {\bf (h)} \\
\end{tabular}}
\end{center}
\vspace{-0.2in}
\caption{Sound wave transformations}
\label{fig:soundwave-transform}
\end{figure*}

\smallskip \noindent
\textbf{Metamorphic Transformations of Sound:} 
\label{sec:meta-trans-methodology}
%A crucial part of 
%software testing is the is oracle problem. We aim to solve this problem by 
%leveraging metamorphic testing. 
\revise{
%In this section, we discuss the transformations applied to speech samples 
%to facilitate the fairness testing embodied in \SMLT. 
The ability to operate in a wide range of environments is crucial in ASR systems 
as they are deployed in safety-critical settings such as medical emergency 
services~\cite{goss2016incidence} and air traffic 
managment~\cite{helmke2016reducing}, \cite{kopald2013applying}, which are 
known to have interference and noise. Metamorphic speech transformations serve to
simulate such scenarios.
The key insight for our metamorphic transformations comes from how 
waves are represented and what can happen to these 
waves when they're transmitted in different mediums.} We realise 
this insight in the fairness testing system for ASR systems. To the 
best of our knowledge \SMLT is the first work that combines this insight 
from \revise{acoustics}, software testing and software fairness 
to evaluate the fairness of ASR systems. 
%
\revise{
\SMLT uses the addition of noise (\Cref{fig:soundwave-transform} (b)),
amplitude modification (\Cref{fig:soundwave-transform} (c)), 
frequency modification (\Cref{fig:soundwave-transform} (d)),
amplitude clipping (\Cref{fig:soundwave-transform} (e)),
frame drops (\Cref{fig:soundwave-transform} (f)), 
low-pass filters (\Cref{fig:soundwave-transform} (g)), and
high-pass filters (\Cref{fig:soundwave-transform} (h)) as metamorphic speech
transformations. We choose these transformations because they are the 
most common distortions for sound in various environments~\cite{kaggleAudio}. 
The details of the transformations are in
\Cref{sec:sound-transformations}.} 


\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.18]{figs/BlockDiagramHorizontal.pdf}
\end{center}
\vspace{-0.2in}
\caption{\SMLT System Overview}
\label{fig:overview}
\vspace{-0.2in}
\end{figure}

\smallskip \noindent
\textbf{System Overview:}
Algorithm~\ref{alg:test-gen} provides an outline of our overall test generation process. 
We realise the notion of fairness described in 
\Cref{eqn:robustness-fairness} using differential testing. The error
rates ($\mathit{ASR}_{Err}$) for a particular speech \revise{clip}
are found by finding the difference 
between the outputs of two ASR systems, ASR$_1$ and ASR$_2$.
It is important to note that we make a design choice to use 
{\em differential testing} to find the error rate ($\mathit{ASR}_{Err}$). 
This helps us eliminate the need for ground truth transcription data which 
is both labor intensive and expensive to obtain.
Furthermore, \SMLT realises the $\delta$ seen in 
\Cref{eqn:robustness-fairness} by using metamorphic transformations 
for speech ({\em see \Cref{fig:overview}}). 
\revise{These speech metamorphic transformations represent the various simulated 
environments for which \SMLT wants to measure the quality of service for different
groups.}
Additionally, the user can customise this $\delta$ per their requirements.
In our implementation we use eight distinct metamorphic transformations
 as $\delta$ 
({\em see \Cref{fig:soundwave-transform}}).
%\SMLT uses 
%the difference in these error rates to find the degradation, and ultimately
%the unfairness in the two ASR systems.
Specifically, we investigate 
how fairly do two ASR systems (ASR$_1$ and ASR$_2$) treat groups
($GR_k^T \mid k \in \{1, 2, \cdots n\}$) with respect to a base group 
($GR_B$). 
\SMLT achieves this by taking a dataset of speech which contains 
data from two or more different groups (e.g. male and female speakers, Native 
English and Non-native English speakers) and modifies these speech snippets 
through a set of transformations ($MT$). These are then divided 
into base group transformed speech ($GR_B^T$) and the 
transformed speech for other groups 
($GR_k^T \mid k \in \{1, 2, \cdots n\}$). 
As seen in \Cref{alg:test-gen}, the average word-level levenshtein 
distance (word-level levenshtein distance divided by the number of words in the longer transcript) between the outputs of the two 
ASR systems is captured by $d_B$ and $d_B^T$ for the original and transformed
speech respectively. 
%\todo{make $d_B$ clearer in text and in the algorithm.}
Similarly, for the comparison groups $GR_k^T (k \in 
\{1, 2, \cdots n\})$ the word-level levenshtein distance is captured by $d_k$ 
and $d_k^T$. The higher the levenshtein distance the larger the error in 
terms of differential testing. In other words, larger error in differential testing 
would mean that the ASR systems disagree on a higher number of words. 

To capture the \revise{degradation in the quality of service} 
for the speech \revise{subjected to simulated environments ($MT$)},
we compute the difference between 
the word-level levenshtein distance for the original and transformed 
speech. Specifically, we compute $D_B$ as $d_B^T - d_B$ and 
$D_k$ as $d_k^T - d_k (k \in 
\{1, 2, \cdots n\})$ for the base and comparison groups, respectively. 
The higher this metric ($D_B$ and $D_k$), the more severe
the degradation in ASR \revise{quality of service} 
because of the transformation~$T$. %\revise{(simulated environment)}.

We compare these metrics and if $D_B$ exceeds $D_k$ by some 
threshold $\tau$, we classify this as an error 
\revise{for the {\em base group} ($GR_B$)} and more specifically a 
violation of fairness ({\em see \Cref{fig:overview}}). In our experiments
we set each of the groups in our dataset as the base group ($GR_B$) and
run the \SMLT technique to find errors with respect to that base group. 
The lower the errors (as computed via the violation of the assertion 
$D_B - D_k \leq \tau$), the fairer the ASR systems are with respect 
to groups $GR_B$. 
%and $GR_k$. 
\revise{As an example, let us say Russian 
speakers are the base group ($GR_B$), English speakers are the 
comparison group ($GR_k$) and the value of $\tau$ is 0.1. If $D_B$ 
is strictly greater than $D_k$ by 0.1, then fairness violation is counted for the Russian 
speakers}. 
\revise{Otherwise, no fairness errors are recorded.}

%If the $D_B$ exceeds $D_k$ by less than or equal to 0.1 or 
%$D_k$ exceeds $D_B$, no error is counted.} 

%Intuitively, \SMLT discovers fairness issues by quantifying the robustness 
%of the speech from a group ($GR_k$) with respect to the the base group 
%$GR_B$ by quantifying the disagreement between two ASR systems. 
%
%
%%The lower the value of $D_k - $ 
%%The lower the errors for the base group, the fairer it is. 
%
%
%
%
%the groups are divided
%into a base group ($GR_B$) and comparison groups 
%($GR_1$, $GR_2$, $\cdots$, $GR_n$). The original speech 
%($GR_B$, $GR_1$, $GR_2$, $\cdots$, $GR_n$) and the corresponding 
%transformations ($GR_B$, $GR_1^T$, $GR_2^T$, $\cdots$, $GR_n^T$) 
%are then processed using the ASR system
%under test. It is important to note that each element in the original 
%speech represents a distinct group.
%The difference between the word error rates (WER) of the 
%output of the ASR system and the ground truth transcript is calculated for 
%the original speech ($O_B$, $O_1$, $O_2$, $\cdots$, $O_n$) and the 
%transformed speech ($O_B^T$, $O_1^T$, $O_2^T$, $\cdots$, $O_n^T$) is 
%calculated ($d_B$, $d_1$, $d_2$, $\cdots$, $d_n$).
%The base group difference ($d_B$) is compared with rest of the groups 
%($d_1$, $d_2$, $\cdots$, $d_n$) and if the difference $d_B - d_k$ 
%where $k \in (1, n)$ is  greater than some user specified threshold $\tau$,
%we consider it a violation in individual fairness and this violation is added
%to the Error Set 
%
%The goal of \SMLT is to show that some groups will have higher differences
%of 
%
% 
%





%\input{Methodology-UserStudy}

\smallskip \noindent
\textbf{Fault Localisation:}
%\todo{Sakshi: Add fault localisation stuff}
%\todo{Test for generality? We use a subset of words shown as erroneous and 
%subset shown as non erroneous. Generate sounds from TTS to show degradation 
%in one and non-degradation in another? Use a grammar to generate words 
%from a TTS?}
%
%
%To aid practitioners using 
\revise{\SMLT introduces a word-level fault
localisation technique, which does not require any access to ground truth 
data}. We first illustrate a use case of this fault localisation technique. 

\smallskip \noindent
\textbf{Example:} Let us consider a corpus of English sentences by a group of 
speakers (say $GR$) who speak language $L_1$ natively. \SMLT builds a dictionary for all 
the words in the transcript obtained from $ASR_1$. An excerpt from such a dictionary 
appears as follows: \{\textit{brother}~:~16, \textit{nice}~:~25, 
\textit{is}~:~33,~$\cdots$\}. This means the words {\em brother, nice} and 
{\em is} were seen 16, 25 and 33 times in the transcript respectively. 
Now, assume \SMLT \revise{simulates a noisy environment}
\revise{
by adding noise with various signal to noise (SNR) ratios as follows: 
\{\textit{10, 8, 6, 4, 2}\}.} This is the parameter for the transformation ($param^T$).

%\SMLT will use noise addition as transformation~($T$) and 
%adds noise with various signal to noise (SNR) ratio: \{\textit{10, 8, 6, 4, 
%2}\}.

Once \SMLT 
obtains the transcript of these transformed inputs, it creates 
dictionaries similar to the ones seen in the preceding paragraph. 
Let the relevant subset of the dictionary for SNR {\em two} (2) be 
\{\textit{brother}~:~1, \textit{nice}~:~23, \textit{is}~:~32,~$\cdots$\}. 
We use this to determine that the utterance
of the word {\em brother} is not robust for noise addition for the group
$GR$. This is because, the word brother appears significantly less in the 
transcript for the modified speech, as compared to the transcript for the 
original speech. 

\begin{algorithm}[t]
	\caption{\SMLT Fault Localizer}
    {\scriptsize
    \begin{algorithmic}[1]
        \Procedure{Fault\_Localizer}
        {$\mathit{WC}$, $\mathit{WC}^{T_{\theta}}$, $\omega$, $param^T$}
        	\State Drop\_Count $\gets \emptyset$ 
        	\State Non\_Robust\_Words $\gets \emptyset$ 
        	
        	\For{$word$ $\in \mathit{WC}.$keys()}
        		\State $init\_count \gets \mathit{WC}[word]$
        		\LineComment Returns the minimum count of $word$ across all 
        		the parameter 
        		\LineComment of transformation $T$ 
        		\State $min\_count \gets$ get\_min($\mathit{WC}^{T_{\theta}}[word]$, 
        		$~param^T$)
        		\State $\mathit{count\_diff} \gets$ max
        		(($init\_count - min\_count)$, 0) 
        		\If{$\mathit{count\_diff} > \omega$}
        			\State Non\_Robust\_Words $\gets$ Non\_Robust\_Words 
        			$~\cup~\{word\}$
        		\EndIf{}
        		
        		\State Drop\_Count $\gets$ Drop\_Count $~\cup~\{count\_diff\}$
        	\EndFor
        	
        	\State \Return {Non\_Robust\_Words, Drop\_Count}
 	\EndProcedure
    \end{algorithmic}
    }
    \label{alg:fault-loc}
 \end{algorithm}





\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.52]{figs/ExplainerBlockDiagram.pdf}
\end{center}
\vspace{-0.2in}
\caption{\SMLT Fault Localization Overview}
\label{fig:fault-loc}
\vspace{-0.2in}
\end{figure}


\smallskip \noindent
\textbf{\SMLT fault localisation overview:}
Algorithm~\ref{alg:fault-loc} provides an overview of the fault localization 
technique implemented in \SMLT. 
The goal of the \SMLT fault localisation is to find words for
a group ($GR$) that are not robust to \revise{
the simulated environments. Specifically, \SMLT finds words which are not 
recognised by the ASR when subjected to the appropriate speech 
transformations.
}

%\revise{the simulated 
%environments. Specifically, \SMLT finds words which are not recognised 
%by the ASR when subjected to the speech transformations that 
%are used to simulate these environment}. 

The transformation 
is represented by $T_{\theta}$. Here, $T \in MT$ is the transformation and 
${\theta} \in param^T$ is the parameter of the transformation, which 
controls \revise{the severity of the transformation.}
%how severely the speech degrades. 

As seen in \Cref{alg:fault-loc},
\SMLT builds a word count dictionary for each word in $WC$ and $WC^{T_{\theta}}$ for 
the original speech and for each ${\theta} \in param^T$ respectively. 
For each word, \SMLT finds the difference in the number of appearances for a 
word in $WC$ and in $WC^{T_{\theta}}$ for ${\theta} \in param^T$. To compute the difference, 
we locate the minimum number of appearances across all the transformation 
parameters ${\theta} \in param^T$ (i.e. $min\_count$ in Algorithm~\ref{alg:fault-loc}). 
This is to locate the worst-case degradation across all transformation parameters. 
The difference is then calculated between $min\_count$ and the number of appearances 
of the word in the original speech (i.e. $init\_count$). If the difference 
exceeds some user-defined threshold $\omega$, then \SMLT classifies the respective 
words as non robust w.r.t the group $GR$ and transformation $T$. 

We envision that practitioners can then review the data generated by fault localization 
(i.e. Algorithm~\ref{alg:fault-loc}) and target the non-robust words to further improve their 
ASR systems \revise{for speech from underrepresented groups~\cite{jain2018improved} and accommodate for speech variability~\cite{huang2001analysis}}. 
In {\bf RQ3}, we validate our fault localization method empirically and in 
{\bf RQ4}, we show how the proposed fault localization method can be used to highlight 
fairness violations.

%\smallskip \noindent
%\textbf{\SMLT unfairness through faults:}
%\todo {Unfairness through fault localisation here or in results?}

%\SMLT then uses the transformation $T_p \in MT$ to build a similar word count
%dictionary $WC^{T_p}$. Here, $p \in param^T$ where $param^T$ is the set of 
%parameters for transformation $T$. For example, if the transformation $T$ 
%is noise addition, the parameters 







==> FASE 2021/motivation.tex <==
\section{Motivation}

\todo{Fairness in ASR}

%BLAH



==> FASE 2021/relatedWork.tex <==
\section{Related Work}

%\smallskip \noindent
%\textbf{Automated Testing of Machine Learning (ML) Systems:}
In the past few years, there has been significant attention in testing 
ML systems \cite{deepXplore,deeptest,deepgauge,deepconcolic,deephunter,tensorfuzz,ogma,checklist,mettle,deepgini,robotDLTesting,calo2020simultaneously,sharma2021mlcheck,Guo2020AAT}. 
Some of these works target coverage-based 
testing~\cite{deeptest,deephunter,tensorfuzz,deepgauge} \revise{or
leverage property driven testing~\cite{sharma2021mlcheck}}, while others focus
effective testing in targeted domains e.g. text~\cite{ogma,checklist}. 
%\revise{
%Others seeks to identify individual discrimination through property driven testing.
%\cite{sharma2021mlcheck}
%}
None of these works, however, are directly applicable for testing ASR systems. 
In contrast, the goal of \SMLT is to automatically discover 
violations of fairness in ASR systems without access to ground truth data. 

%
%One of the first works in this field was 
%Deeptest~\cite{deeptest} which leveraged metamorphic behaviour to 
%identify erroneous behaviours in an ML model. DeepXplore~\cite{deepXplore} 
%is a white-box differential testing
%algorithm which aims to find inputs that can trigger inconsistencies
%between multiple deep neural networks (DNNs).
%DeepGauge~\cite{deepgauge} formalises a multi-granularity testing coverage 
%criteria for testing DNNs and measures the testing quality.
%DeepConcolic~\cite{deepconcolic} aims to discover violations of robustness.
%and to this end, it builds a framework to perform concolic testing on ML 
%systems. DeepHunter~\cite{deephunter} and TensorFuzz~\cite{tensorfuzz} 
%focus on coverage guided fuzzing for ML systems.
%Ogma~\cite{ogma} and CheckList~\cite{checklist} focus on functional 
%and behavioural testing for NLP systems respectively. METTLE~\cite{mettle} 
%develops a metamorphic testing approach to test unsupervised learning 
%sytems. DeepGini~\cite{deepgini} and RobOT~\cite{robotDLTesting}
%build tests with the aim to enhance the robustness of the ML models 
%under test. 
%
%In contrast to these works, the goal of \SMLT to automatically discover 
%violations of fairness in automated speech recognition systems without
%access to ground truth data. 

%Deeptest~\cite{deeptest}, deepXplore~\cite{deepXplore}, 
%deepconconcolic~\cite{deepconcolic}, mettle~\cite{mettle}, 
%deephunter~\cite{deephunter}, tensorfuzz~\cite{tensorfuzz}, Ogma~\cite{ogma}, checklist~\cite{checklist}, deepgini~\cite{deepgini}
%robot~\cite{robotDLTesting}. 

%\todo{Copy paste argument from Astraea about explainability}




%\smallskip \noindent
%\textbf{ASR Testing and Adversarial Attacks:}
%To the best of our knowledge only two works have been proposed for 
%the testing of mature ASR systems, namely DeepCruiser~\cite{deepcruiser} 
%and CrossASR~\cite{crossASR}. 
%DeepCruiser~\cite{deepcruiser} uses metamorphic transformations
%and performs coverage-guided fuzzing with the goal of generating 
%audio that has errors in the transcript produced by the ASR system. 
%Concurrently, CrossASR~\cite{crossASR} uses text to generate speech from a TTS engine 
%and subsequently employs differential testing to find bugs in the ASR 
%system. 
DeepCruiser~\cite{deepcruiser} uses metamorphic transformations
and performs coverage-guided fuzzing to discover transcription errors 
in ASR systems. Concurrently, CrossASR~\cite{crossASR} uses text to 
generate speech from a TTS engine and subsequently employs differential 
testing to find bugs in the ASR system.
In contrast to these systems, the goal of \SMLT is to automatically find
violations of fairness by measuring the degradation of transcription 
quality from the ASR when the speech is transformed. \SMLT compares 
this degradation across various groups of speakers and if the 
difference is substantial, \SMLT characterises this as a fairness
violation. 
%\revise{
Moreover, \SMLT neither requires access 
to manually labelled speech data nor does it require any white/grey box 
access to the ASR model.
%} 
%
%There are also works that craft adversarial examples for specific snippets 
%of speech~\cite{automatedBasicRecognition}, \cite{fakeBob}, 
%\cite{audioAdversarial}, \cite{imperceptibleASRadversarial}, 
%\cite{foolingAsr}. 
%The goal of these works is to find
%an imperceptible perturbation that are specially crafted for an audio file
%which causes an error in the transcription. On the other hand, \SMLT aims 
%to find fairness violations. Specifically, \SMLT aims to discover if two groups
%whose speech have similar performance on the surface, perform vastly 
%differently when the speech is modified. Additionally, to the best of our
%knowledge, \SMLT is the first technique to propose automatic fault 
%localisation for ASR systems without the use of a ground truth transcript. 
%
Works on audio adversarial testing~\cite{automatedBasicRecognition}, 
\cite{fakeBob}, \cite{audioAdversarial}, \cite{imperceptibleASRadversarial}, 
\cite{foolingAsr} aims to find
an imperceptible perturbation that are specially crafted for an audio file. 
In contrast, \SMLT aims to find fairness violations. Additionally, \SMLT 
also proposes automatic fault 
localisation for ASR systems without using a ground truth transcript.

%Deepcruiser~\cite{deepcruiser}, crossasr~\cite{crossASR}

%Audio Adversarial~\cite{audioAdversarial}, fooling 
%end-to-end~\cite{foolingAsr}, imperceptiple 
%asr~\cite{imperceptibleASRadversarial}
%automated basic recognition test~\cite{automatedBasicRecognition}

%\smallskip \noindent
%\textbf{Fairness in ML:}
%Themis~\cite{themis}, Ignorance~\cite{ignoranceAndPrejudice}, blackbox 
%fairness~\cite{blackboxFainess}, whiteBox~\cite{whiteboxFairness}, 
%astraea~\cite{astraea}
%
\revise{Unlike \SMLT, recent works on fairness testing have focused 
on credit rating~\cite{themis,aequitas,blackboxFainess,ignoranceAndPrejudice,sharma2019testing,sharma2020higher,sharma2020automatic,sharma2021mlcheck}, 
computer vision~\cite{denton2019image,buolamwini2018gender} or NLP systems~\cite{ijcai_nlp_testing,astraea}.
In the systems that deal with such data, it is possible to isolate certain
sensitive attributes (gender, age, nationality) and test for 
fairness based on these attributes. It is challenging to isolate such 
sensitive attributes in speech data, necessitating the need for a separate
fairness testing framework specifically for speech data.}
%\SMLT formalises and automates the 
%fairness testing of ASR systems and localizes faults at the input level.}

%Recent approaches on fairness 
%testing~\cite{themis}, \cite{aequitas}, \cite{ignoranceAndPrejudice}, 
%\cite{whiteboxFairness}, \cite{ijcai_nlp_testing}, \cite{blackboxFainess}, 
%\cite{astraea} are not directly applicable for fairness testing of ASR 
%systems. These approaches are mostly focused on the
%fairness testing of credit rating, computer vision systems or NLP systems.
%In contrast to these approaches, \SMLT formalises and automates the 
%fairness testing of ASR systems. To the best of our knowledge, \SMLT 
%is the first work that automates the fairness testing of ASR systems and 
%localises the faults to better guide practitioners. 

%\smallskip\noindent
%\textbf{Explainable AI:} 
%\revise{
Frameworks such as LIME~\cite{lime}, SHAP~\cite{shap}, Anchor~\cite{anchor} and DeepCover~\cite{eccv2020_fault}
attempt to reason why a model generates a specific
output for a specific input.
In contrast to this, \SMLT's fault localisation algorithm 
identifies utterances spoken 
by a group which are likely to be not recognised by ASR systems in the 
presence of a destructive interference (such as noise).
%In contrast, an explanation-based framework (such as 
%LIME~\cite{lime}) solves an orthogonal problem: to reason why a model generates a specific output for an input?}
\revise{Recent fault localization approaches either aim to  
%minimal set of 
%features explaining the outputs of image classifiers~\cite{eccv2020_fault} or they 
highlight the neurons~\cite{fase2019_fault} or training code~\cite{icse2021_fault} 
that are responsible for a fault during inference. 
In contrast, \SMLT highlights words that are likely to be transcribed wrongly without 
having any access to the ground truth transcription and with only blackbox access to 
the ASR system.} 

%\revise{
%LIME~\cite{lime} builds linear classifiers to explain the behaviour of 
%the prediction of a given ML model and Anchor~\cite{anchor} tries to 
%do the same using if-then rules called anchors. 
%SHAP~\cite{shap} leverages Shapely values from game theory for 
%an approach which connects local explanations to optimal 
%credit allocations.
%Another work~\cite{contrastiveExplanation} utilises structural causal 
%models~\cite{structuralCausalExplanation} to explain models 
%using contrastive explanations. Unlike these works, the fault localization 
%of \SMLT aims to identify the non-robust words contributing to an error.  
%Specifically, LIME~\cite{lime} explains the predictions of a classifier 
%by trying to understand the behaviour of the prediction around a given 
%classifier locally using linear classifiers. Meanwhile,  Anchor~\cite{anchor} 
%explains classifier predictions via if-then rules called anchors. 
%SHAP~\cite{shap} employs a game theoretic approach to explain the output
%of a model by connecting optimal credit allocations with local 
%explanations. This is done using Shapely values from game theory. 
%Another recent work~\cite{contrastiveExplanation} seeks to explain models
%using contrastive explanations based on structural causal 
%models~\cite{structuralCausalExplanation}.
%\todo{Discuss LIME, SHAP, Anchor, Contrastive Explanation for 
%generating local failure reasons}
%}


%Fairspeech~\cite{racialASR}





==> FASE 2021/results.tex <==
\section{Results}
\label{sec:results}
\smallskip
In this section, we discuss our evaluation of \SMLT in detail. In particular, 
we structure our evaluation in the form of four research questions 
({\bf RQ1} to {\bf RQ4}). The analysis of these research questions appears in the 
following sections. 


%\begin{figure}[t]
%\begin{center}
%\includegraphics[scale=0.2]{{figs/Accents-Total-Errors.png}}
%\end{center}
%\caption{Total errors in the Accents dataset}
%\label{fig:accents-total-errors}
%%\vspace{-0.2in}
%\end{figure}
%\begin{figure*}[t]
%\begin{center}
%\begin{tabular}{ccc}
%\includegraphics[scale=0.2]{figs/Accents-Total-Errors.png} &
%\includegraphics[scale=0.2]{figs/Accents-Tau-Errors.png} & 
%\includegraphics[scale=0.2]{{figs/Accents-ASR-Errors.png}} \\
%{\bf (a)} & {\bf (b)} & {\bf (c)} \\
%\includegraphics[scale=0.2]{figs/Accents-Transition-1-Errors.png} & 
%\includegraphics[scale=0.2]{figs/Accents-Transition-2-Errors.png} & 
%\includegraphics[scale=0.2]{figs/Accents-Transition-3-Errors.png} 
% \\
% {\bf (d)} & {\bf (e)} & {\bf (f)} \\
%\end{tabular}
%
%\end{center}
%\caption{Sensitivity analysis for the Accents dataset}
%\label{fig:accents-errors}
%\end{figure*}
%
%
\smallskip \noindent
\textbf{\revise{RQ1: What is \SMLT's efficacy?}} 
%In this section we discuss the efficacy of \SMLT's error generation. 

We structure the analysis of this research question into three sections, 
each corresponding to a dataset we have used in our analysis. 
\revise{All of the relevant data is presented in \Cref{tab:smlt-errors}.}
%
We first analyse the number of errors (used interchangeably with fairness
violations) for each case. Subsequently, we 
analyse the sensitivity of the errors with respect to the values of 
$\tau$ ($\tau \in $ \{0.01, 0.05, 0.1, 0.15\}). 
\revise{Detecting violations of fairness is regulated by parameter $\tau$. Lower values of $\tau$ imply that the degradation of word error rates between two groups should be similar, and conversely higher values of $\tau$ allow for the difference in degradation of word error rates to be more severe between two groups.}
%\todo {Mention Rationale for excluding the 2 least comprehensible Scale transformations.}
Next, we analyse the sensitivity of the pairs of the ASR systems under test. 
Concretely, we analyse the errors found in the  Microsoft Azure and IBM Watson 
{\em (MS\_IBM)}, Google Cloud and IBM Watson {\em (IBM\_GCP)}, and Microsoft 
Azure and Google Cloud {\em (MS\_GCP)} pairs. Finally, we analyse the sensitivity 
of the \SMLT test generation with respect to the eight different types of transformations 
implemented (see \Cref{fig:soundwave-transform}).

It is important to note that that we excluded the two 
most destructive Scale transformations. This is because the word error rate 
for these transformations is 0.89 on average out of 1. This degradation may 
be attributed to the transformation itself rather than the ASR. 
To avoid such cases, we exclude these transformations from this 
research question.%}


\begin{table*}[t]
\caption{Errors Discovered by \SMLT}
\centering
	\resizebox{\linewidth}{!}{
    \begin{tabular}{lr rrrrrrr rrr rr}
        \toprule
        \multicolumn{1}{l}{}  & \multicolumn{7}{c} {Accents} & \multicolumn{2}{c} {RAVDESS} & \multicolumn{2}{c} {\makecell{Nigerian/Midlands\\English}} \\ \cmidrule(lr){2-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12}
        \multicolumn{1}{l}{}  & English & Ganda & French & Gujarati & 
        Indonesian &	Korean & 	Russian &  Male & Female & Midlands & Nigerian \\ \midrule
        
        \textbf{Total Errors} & 312 &	844 &	413 &
        406 &	311 & 1086	& 853 & 28 & 176 & 93 & 239\\
        \textbf{$\tau$ Sensitivity}  \\
         \multicolumn{1}{r}{\textit{0.01}} & 168 & 381 & 267 & 232 & 178 & 499 & 354 & 12 & 92  & 36 & 75 \\
		 \multicolumn{1}{r}{\textit{0.05}} & 75 & 245 & 99 & 101 & 85 & 340 & 227 & 8 & 53 & 26 & 65 \\
		 \multicolumn{1}{r}{\textit{0.10}} & 43 & 145 & 39 & 49 & 34 & 172 & 161 & 5 & 21 & 17 & 55\\ 
		 \multicolumn{1}{r}{\textit{0.15}} & 26 & 73 & 8 & 24 & 14 & 75 & 111 & 3 & 10 & 14 & 44\\ 
		 \textbf{ASR Sensitivity} \\
		 \multicolumn{1}{r}{\textit{MS IBM}} & 36 & 369 & 128 & 126 & 64 & 388 & 303 & 10 & 57 & 30 & 86 \\
\multicolumn{1}{r}{\textit{GCP IBM}} & 131 & 325 & 123 & 147 & 98 & 342 & 361& 9 & 64 & 31 & 96\\ 
\multicolumn{1}{r}{\textit{MS GCP}} & 145 & 150 & 162 & 133 & 149 & 356 & 189 & 9 & 55 & 32 & 57\\
		\textbf{Transition Sensitivty} \\
		\multicolumn{1}{r}{\textit{Clipping}} & 4 & 81 & 38 & 159 & 72 & 182 & 237 & 0 & 24 & 50 & 3\\
		\multicolumn{1}{r}{\textit{Drop}} & 8 & 113 & 33 & 29 & 40 & 184 & 45 & 0 & 21 & 4 & 33  \\
		\multicolumn{1}{r}{\textit{Frame}} & 14 & 106 & 61 & 25 & 36 & 170 & 26 & 1 & 13 & 13 & 19\\
		\multicolumn{1}{r}{\textit{Noise}} & 5 & 128 & 54 & 86 & 22 & 217 & 213& 0 & 24 & 5 & 43 \\
		\multicolumn{1}{r}{\textit{LP}} & 39 & 158 & 108 & 57 & 14 & 110 & 208 & 0 & 45 & 4 & 34  \\
		\multicolumn{1}{r}{\textit{Amplitude}} & 81 & 19 & 44 & 33 & 14 & 40 & 26 & 0 & 27 & 8 & 40\\
		\multicolumn{1}{r}{\textit{HP}} & 114 & 168 & 29 & 9 & 61 & 87 & 57 & 9 & 20 & 1 & 51  \\
		\multicolumn{1}{r}{\textit{Scale}} & 47 & 71 & 46 & 8 & 52 & 96 & 41 & 18 & 2 & 8 & 16 \\
%        \multicolumn{2}{l}{Microsoft (MS)} & \\
%        & \textit{Robust} & 99 & \multirow{8}{*}{\makecell{Looking\\Good}} &  
%        \multirow{8}{*}{\makecell{Very\\Clear}}\\ 
%        & \textit{Non-Robust} & 99 & &  \\ 
%        1
%        \multicolumn{2}{l}{Google Cloud (GCP)} & \\
%         & \textit{Robust} & 100 &  & \\ 
%        & \textit{Non-Robust} & 99 & & \\ 
%        \cmidrule{1-3}
%        \multicolumn{2}{l}{IBM Watson (IBM)} & \\
%        & \textit{Robust} & 100 & &  \\ 
%        & \textit{Non-Robust} & 96 & & \\ 
        \bottomrule
    \end{tabular}}
    \label{tab:smlt-errors}
\end{table*}

%\todo{Sakshi has removed all (see \Cref{tab:smlt-errors}) because too much repetition}

\smallskip \noindent
\textbf{Accents Dataset:}
%\Cref{tab:smlt-errors} (Accents) 
%shows all the errors found by \SMLT for the 
%speech accents dataset~\cite{accents}. This 
%includes all transformations, all values of $\tau$ (0.01, 0.05, 0.1, 0.15) and all the ASR systems 
%under test. 
Native English speakers and Indonesian speakers have the lowest 
number of errors. 
%
%found followed by native French and Gujarati speakers. 
%Native Ganda, Russian and Korean speakers have the most errors and tend to be 
%the least robust. 
On average, speech from non-native English speakers 
generates {\em 109\% more errors} in comparison to speech from native 
English speakers. 
%
%\begin{figure}[t]
%\begin{center}
%\includegraphics[scale=0.2]{{figs/Accents-Tau-Errors.png}}
%\end{center}
%\caption{Errors in the Accents dataset ($\tau$ sensitivity)}
%\label{fig:accents-tau-errors}
%%\vspace{-0.2in}
%\end{figure}
%
For the two smallest values of $\tau$, speech from the native 
English speakers \revise{shows the {\em least number} of fairness violations}.
%(\textit{see \Cref{tab:smlt-errors}}). 
%This means speech from native English 
%speakers is the most robust when the tolerance is low. 
%As the value of $\tau$ 
%increases so does the tolerance to the errors speech from Ganda, Korean and 
%Russian speakers still performs significantly worse than speech from English 
%speakers. 
%\revise {
%As the value of $\tau$ 
%increases, so does the tolerance to the errors. Speech from native Ganda, Korean 
%and Russian speakers still performs significantly worse than speech from English 
%speakers.
%} 
%On average, speech from non-native English speakers generate 
%89.5\%, 143.7\%, 132.5\%, 95.5\% more errors than native English 
%speakers for $\tau$ $\in$ (0.01, 0.05, 0.1, 0.15) respectively. 
%
Speech from native English speakers has the lowest, second lowest and third 
lowest errors for the pairs of ASRs, {\em(MS\_IBM)}, {\em(MS\_GCP)} and 
{\em(IBM\_GCP)} respectively. 
%(\textit{see \Cref{tab:smlt-errors}}). 
%On average non-English speakers generate 537.9\%, 30.9\% and 77.6\% more 
%errors than English speakers for {\em(MS\_IBM)}, {\em(MS\_GCP)} and 
%{\em(GCP\_IBM)} respectively.
%
Speech from native English speakers has the lowest errors for the 
clipping, two types of frame drops and noise transformations and the second 
lowest errors for the low-pass filter transformation.
%(\textit{see \Cref{tab:smlt-errors}}). 
%Speech from non-native 
%English speakers has 3104.6\%, 825\%, 404\%, 2300\% and 179\% more errors 
%on average than speech from native English speakers for the
%clipping, drop, frame, noise and low-pass filter transformations 
%respectively. 
The remaining transformations, namely amplitude, high-pass filter and 
scaling induce a comparable number of errors from native and 
non-native English speakers.
%(\textit{see \Cref{tab:smlt-errors}}). 
%Speech from non-native 
%English speakers on average generates less errors in amplitude (63.7\%) and 
%high-pass filters (39.9\%) and only slightly more (11.3\%) in comparison
%to native English speakers.

\begin{result}
Speech from non-native English speakers generally 
\revise{exhibits more fairness violations in} 
comparison to speech from native English speakers.
\end{result}
%
%\begin{figure}[t]
%\begin{center}
%\includegraphics[scale=0.2]{{figs/Accents-ASR-Errors.png}}
%\end{center}
%\caption{Errors in the Accents dataset (ASR sensitivity)}
%\label{fig:accents-asr-errors}
%%\vspace{-0.2in}
%\end{figure}



%\begin{figure}[t]
%\begin{center}
%\includegraphics[scale=0.2]{{figs/RAVDESS-Total-Errors.png}}
%\end{center}
%\caption{Total errors in the RAVDESS dataset}
%\label{fig:ravdess-total-errors}
%%\vspace{-0.2in}
%\end{figure}
%
%\begin{figure}[t]
%\begin{center}
%\includegraphics[scale=0.2]{{figs/RAVDESS-Tau-Errors.png}}
%\end{center}
%\caption{Errors in the RAVDESS dataset ($\tau$ sensitivity)}
%\label{fig:ravdess-tau-errors}
%%\vspace{-0.2in}
%\end{figure}

%\begin{figure*}[t]
%\begin{center}
%\begin{tabular}{ccc}
%\includegraphics[scale=0.2]{figs/RAVDESS-Total-Errors.png} &
%\includegraphics[scale=0.2]{figs/RAVDESS-Tau-Errors.png} & 
%\includegraphics[scale=0.2]{figs/RAVDESS-ASR-Errors.png} \\
%{\bf (a)} & {\bf (b)} & {\bf (c)} \\
%\includegraphics[scale=0.2]{figs/RAVDESS-Transition-1-Errors.png} & 
%\includegraphics[scale=0.2]{figs/RAVDESS-Transition-2-Errors.png} & 
%\includegraphics[scale=0.2]{figs/RAVDESS-Transition-3-Errors.png} 
% \\
% {\bf (d)} & {\bf (e)} & {\bf (f)} \\
%\end{tabular}
%
%\end{center}
%\caption{Sensitivity analysis for the RAVDESS dataset}
%\label{fig:ravdess-errors}
%\end{figure*}

\smallskip \noindent
\textbf{RAVDESS Dataset:}
%\Cref{tab:smlt-errors} (RAVDESS) 
%shows all the errors found by \SMLT for the 
%RAVDESS dataset~\cite{ravdess}. This 
%includes all transformations, all values of $\tau$ (0.01, 0.05, 0.1, 0.15) 
%and all the ASR systems under test. 
Speech from male speakers has significantly 
lower errors than speech from female speakers.
%(\textit{see \Cref{tab:smlt-errors}}). 
On average, speech from female speakers 
generates {\em 528.57\% more errors} in comparison to speech from male speakers.
%
%
%For all values of $\tau$, speech from the male speakers is the most robust. 
%(\textit{see \Cref{tab:smlt-errors}}).
%This means speech from male speakers is more robust than speech from female 
%speakers for all tolerances in our experimentation. 
%Speech from female speakers generates 666.6\%, 562.5\%, 323\%, 233.3\% more 
%errors than speech from male speakers, on average for $\tau$ $\in$ 
%(0.01, 0.05, 0.1, 0.15) respectively.
%
%Speech from male speakers is significantly more robust for all ASR pairs
%tested.
\revise{
Speech from male speakers \revise{shows significantly fewer fairness violations} 
for all values of $\tau$, and for all ASR pairs tested.}
%(\textit{see \Cref{tab:smlt-errors}}). 
%On average speech from female speakers generates 470\%, 611.1\% and 511.1\% more errors than speech from male speakers for {\em(MS\_IBM)}, 
%{\em(GCP\_IBM)} and {\em(MS\_GCP)} respectively.
\revise{
Clipping, both types of frame drops, noise, low-pass and
amplitude induce significantly fewer errors on speech from male
speakers.}
%Speech from male speakers does not have errors for the 
%clipping, one type of frame drop, noise, low-pass and amplitude 
%transformations and only one error for the other type of frame drop. 
%In contrast, speech from female speakers has significantly more errors. 
%(\textit{see \Cref{tab:smlt-errors}}). 
%
However, speech from both groups have comparable number of errors when
subject to high-pass and scale transformations. 

\begin{result}
Speech from female speakers \revise{has significantly higher fairness violations} in 
comparison to speech from male speakers.
\end{result}

\smallskip \noindent
\textbf{Midlands/Nigeria Dataset:}
%\Cref{tab:smlt-errors} (Nigerian/Midlands English) 
%shows all the errors found by \SMLT for 
%the UK Midlands dataset~\cite{uk-midlands-dataset} compared to the Nigerian 
%English dataset~\cite{nigerian-english}. This 
%includes all transformations, all values of $\tau$ (0.01, 0.05, 0.1, 0.15) 
%and all the ASR systems under test. 
Speech from UK Midlands English (ME)
speakers has significantly lower errors 
than speech from Nigerian English (NE) speakers.
%(\textit{see \Cref{tab:smlt-errors}}). 
On average, speech from NE speakers
generates {\em 156.9\% more errors} in comparison to speech from 
ME speakers.
%
%
\revise{
Speech from ME speakers has significantly fewer fairness errors for all values of $\tau$, 
and for all ASR pairs tested.}
%For all values of $\tau$, speech from ME 
%speakers is more robust than speech from NE speakers. 
%(\textit{see \Cref{tab:smlt-errors}}).
%\todo{Check}
%This means speech from ME speakers is 
%more robust than speech from NE speakers 
%for all tolerances in our experimentation. 
%Speech from Nigerian English speakers generates 108.3\%, 150\%, 223.5\%, 214.23\% more 
%errors than speech from UK Midlands English 
%speakers, on average for $\tau$ $\in$ 
%(0.01, 0.05, 0.1, 0.15) respectively.
%
%Speech from ME speakers is significantly 
%more robust for all ASR pairs tested. 
%(\textit{see \Cref{tab:smlt-errors}}). 
%On average speech from Nigerian English speakers 
%generates 186.6\%, 209.66\% and 78.12\% 
%more errors than speech from UK Midlands English 
%speakers for {\em(MS\_IBM)}, {\em(GCP\_IBM)} and {\em(MS\_GCP)} respectively.
%
For the transformations scale, drop, noise, amplitude, low pass and high pass 
filters, the speech from ME speakers has significantly 
fewer error than speech from NE speakers.
%(\textit{see \Cref{tab:smlt-errors}}). 
%Speech from Nigerian 
%English speakers generates, on average 100\%, 725\%, 760\%, 400\%, 5000\% and
%750\% more errors than speech from UK Midlands English speakers for 
%scale, drop, noise, amplitude, low pass and high pass filter transformations
%respectively. 
For the transformations, clipping and frame, we find that speech from both 
groups have similar number of errors.

\begin{result}
Speech from Nigerian English speakers
\revise{has significantly more fairness errors} in 
comparison to speech from UK Midlands speakers.
\end{result} 


%\begin{figure*}[t]
%\begin{center}
%\begin{tabular}{cccccc}
%\includegraphics[scale=0.2]{figs/Nigeria_UK_Midlands-Total-Errors.png} &
%\includegraphics[scale=0.2]{figs/Nigeria_UK_Midlands-Tau-Errors.png} & 
%\includegraphics[scale=0.2]{figs/Nigeria_UK_Midlands-ASR-Errors.png}  \\
%{\bf (a)} & {\bf (b)} & {\bf (c)} \\
%\includegraphics[scale=0.2]{figs/Nigeria_UK_Midlands-Transition-1-Errors.png} & 
%\includegraphics[scale=0.2]{figs/Nigeria_UK_Midlands-Transition-2-Errors.png} & 
%\includegraphics[scale=0.2]{figs/Nigeria_UK_Midlands-Transition-3-Errors.png} 
%\\
%{\bf (d)} & {\bf (e)} & {\bf (f)} \\
%\end{tabular}
%
%\end{center}
%\caption{Sensitivity analysis for the Nigerian English/UK Midlands English dataset}
%\label{fig:nigeria-midlands-errors}
%\end{figure*}


%\begin{table}
%\caption{More }
%\centering
%    \begin{tabular}{lp{6cm}}
%        \toprule
%        Test \\ \midrule
%%        Notation & Description \\ \midrule
%%	    $GR_B$ & Base group  \\
%%	    $GR_k$ & $k \in (1, n)$. Various comparison group  \\
%%	    $MT$ & Metamorphic transformations \\
%%	    $ASR$ & Automatic Speech Recognition system under test \\
%%	    $\tau$ &  A user specified threshold beyond which the difference in 
%%	    word error rate for the base and comparison groups is considered 
%%	    an violation of individual fairness\\
%%        \bottomrule
%    \end{tabular}
%    \label{tab:error-inc-english}
%\end{table}






%
%\begin{figure}[t]
%\begin{center}
%\includegraphics[scale=0.3]{{figs/Accents-Total-Errors.png}}
%\end{center}
%\caption{Total errors in the Accents dataset}
%\label{fig:accents-total-errors}
%%\vspace{-0.2in}
%\end{figure}

\smallskip \noindent
\textbf{RQ2: What are the effects of transformations on 
comprehensibility?}



To better understand the effects of the transformations (\textit{see 
\Cref{fig:soundwave-transform}}) on the 
comprehensibility of the speech we conducted a user study. 
\revise{Speech of one {\em female native English} speaker from the 
Accents~\cite{accents} dataset was used. Survey participants 
were presented with the 
original audio file along with a set of transformed speech files in 
order of increasing intensity. All the transformations ({\em see 
\Cref{fig:soundwave-transform}}) and transformation parameters ({\em see 
\Cref{tab:transList}}) were used.}
We asked 200 survey participants (\revise{sourced through Amazon mTurk}) 
the following question:
\begin{result}
{\fontfamily{qcr}\selectfont
How comprehensible is (transformed) Speech with respect to the 
Original speech?}
\end{result}

\begin{wrapfigure}{l}{0.44\textwidth}
%\begin{figure}[t]
\vspace{-0.2in}
\begin{center}
\includegraphics[scale=0.37]{figs/User-Study-Graph.png}
\end{center}
\vspace{-0.2in}
\caption{Average Transformation Comprehensibility Ratings}
\label{fig:user-study-results}
\vspace{-0.2in}
%\end{figure}
\end{wrapfigure} 

The rating of one (1) is {\em Not Comprehensible at all} and the rating 
of ten (10) is {\em Just as Comprehensible as the Original}.

%\todo {Add full average drop tables to appendix?}



Unsurprisingly, as seen in \Cref{fig:user-study-results}, increasing 
the intensities of the transformation had a generally detrimental effect on
the comprehensibility of the speech. But none of the transformations 
majorly affect the comprehensibility of the speech. All of the 
transformations had a \revise{average} comprehensibility rating above 6.75 and 82.9\%
of the transformations had a comprehensibility rating above 7.



%\begin{wrapfigure}{l}{0.5\textwidth}
%%\begin{figure}[t]
%\vspace{-0.2in}
%\begin{center}
%\includegraphics[scale=0.42]{figs/User-Study-Graph.png}
%\end{center}
%\caption{Average Transformation Comprehensibility Ratings}
%\label{fig:user-study-results}
%\vspace{-0.2in}
%%\end{figure}
%\end{wrapfigure}

The average degradation in comprehensibility for the least 
destructive parameter across all transformations was 24.36\%. Noise
was the most destructive at 27.75\% and drop was the least
destructive (20.96\%). 

The average degradation in comprehensibility for the most 
destructive parameter across all transformations was 29.18\%. In this 
case, scaling 
was the most destructive at 32.23\% whereas drop was the least
destructive with 25.88\%. 

Additionally, for each transformation, we analyse the percentage 
drop of comprehensibility between the least and the most 
destructive transformation parameters. The average drop is 4.82\% 
across all transformations. The scaling and drop transformations 
show high relative percentage drops of 10.05\% and 8.32\% respectively. 
Amplitude, clipping, noise, high-pass and low-pass filters show closer 
to average drops between 3.1\% and 4.5\%. Frame, on the other hand, 
shows very low relative drops at 0.76\%.

\begin{result}
All the transformations, though destructive, are comprehensible by humans. 
\end{result}




For safety critical applications, we recommend that future work test the 
whole gamut of transformations. For other use cases, practitioners may choose
the transformations that satisfy their needs. 
To aid this, \SMLT allows the users to choose the comprehensibility 
threshold of the transformations. As seen in \Cref{tab:rq2-errors-compre}, 
our conclusion holds even if we choose the transformations with higher comprehensibility 
threshold (7.2). In particular, we observe that speech from native English speakers, 
male and UK Midlands Speakers generally exhibit lower errors. 
The detailed sensitivity analysis for the errors is seen in 
\Cref{fig:accents-errors-comp-thresh-7-2}, 
\Cref{fig:ravdess-errors-comp-thresh-7-2} and
\Cref{fig:nigeria-midlands-errors-comp-thresh-7-2} in the appendix. 
Additional user study details are seen in \Cref{sec:user-study-details}.
%\revise {Should the error images for the breakdown be included in the
%appendix?}





%\begin{figure*}[t]
%\begin{center}
%\resizebox{\linewidth}{!}{
%\begin{tabular}{ccc}
%\includegraphics[scale=0.2]{figs/RQ2/Accents-Total-Errors-Comprehensibility-Thresh-7_2.png} &
%\includegraphics[scale=0.2]{figs/RQ2/RAVDESS-Total-Errors-Comprehensibility-Thresh-7_2.png} &
%\includegraphics[scale=0.2]{figs/RQ2/Nigeria_UK_Midlands-Total-Errors-Comprehensibility-Thresh-7_2.png} \\
%\\
%{\bf (a)} & {\bf (b)} & {\bf (c)}\\
%\end{tabular}}
%\caption{Unfairness errors where the transformations have a comprehensibility rating of at least 7.2}
%\end{center}
%\label{fig:rq2-errors-compre}
%%\vspace{-0.2in}
%\end{figure*}

\begin{table*}[t]
\caption{Fairness errors where the transformations have a comprehensibility rating of at least 7.2}
\centering
	\resizebox{\linewidth}{!}{
    \begin{tabular}{lr rrrrrrr rrr rr}
        \toprule
        \multicolumn{1}{l}{}  & \multicolumn{7}{c} {Accents} & \multicolumn{2}{c} {RAVDESS} & \multicolumn{2}{c} {\makecell{Nigerian/Midlands English}} \\ \cmidrule(lr){2-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12}
        \multicolumn{1}{l}{}  & English & Ganda & French & Gujarati & 
        Indonesian &	Korean & 	Russian &  Male & Female & Midlands & Nigerian \\ \midrule
        
        \textbf{\makecell{Total Errors}} & 246 &	509 &	240 &
        166 &	225 & 687	& 329 & 28 & 88 & 55 & 161\\
        \bottomrule
    \end{tabular}}
    \label{tab:rq2-errors-compre}
\end{table*}

\begin{table}[t]
\caption{Grammar-generated sentence examples}
\centering

\resizebox{\linewidth}{!}{\scriptsize
	\begin{tabular}{lrp{4cm}p{4cm}p{4cm}}
	\toprule
	 \multicolumn{2}{l}{ASR}  & \multicolumn{1}{l}{Microsoft} 
	 &\multicolumn{1}{l}{Google Cloud} 
	 & \multicolumn{1}{l}{IBM Watson} \\ \midrule
	 & \textit{Robust} & Ashley likes \textbf{fresh} smoothies & Karen loves \textbf{plastic} straws & William detests \textbf{plastic} cups\\ 
     & & Paul adores \textbf{spoons} of cinnamon & Donald hates 
     \textbf{big} decisions & Steven detests \textbf{big} flags  \\ \\
     & \textit{Non-robust}  &  Ashley detests \textbf{thick} smoothies &
     John loves \textbf{spoons} of cinnamon &
     Betty likes \textbf{scoops} of ice cream \\ 
     & & Ryan likes \textbf{slabs} of cake  & Robert loves \textbf{bags} 
     of concrete & Amanda is fond of \textbf{things} like groceries   \\ 
	 \bottomrule
	\end{tabular}

}
\label{tab:gram-sentences}
\end{table}
%\begin{table}[t]
%\caption{Example grammar-generated sentences}
%\centering
%	{\scriptsize
%    \begin{tabular}{lrp{4cm}}
%        \toprule
%        \multicolumn{2}{l}{ASR}  & Sentence Example \\ \midrule
%        \multicolumn{2}{l}{Microsoft (MS)} & \\
%        & \textit{Robust} & Ashley likes \textbf{fresh} smoothies \\ 
%        & & Paul adores \textbf{spoons} of cinnamon \\ \\
%        & \textit{Non-robust}  &  Ashley detests \textbf{thick} smoothies \\ 
%        & & Ryan likes \textbf{slabs} of cake \\ 
%        \midrule
%        \multicolumn{2}{l}{Google Cloud (GCP)} & \\
%		& \textit{Robust} & Karen loves \textbf{plastic} straws \\ 
%        & & Donald hates \textbf{big} decisions \\ \\
%        & \textit{Non-robust}  & John loves \textbf{spoons} of cinnamon \\ 
%        & & Robert loves \textbf{bags} of concrete \\ 
%        \midrule
%        \multicolumn{2}{l}{IBM Watson (IBM)} & \\
%        & \textit{Robust} & William detests \textbf{plastic} cups \\
%        & & Steven detests \textbf{big} flags \\ \\
%         & \textit{Non-robust}  & Betty likes \textbf{scoops} of ice cream \\
%         & & Amanda is fond of \textbf{things} like groceries  \\
%        \bottomrule
%    \end{tabular}}
%    \label{tab:gram-sentences}
%\end{table}

\smallskip \noindent
\textbf{RQ3: Are the outputs produced by \SMLT fault localiser 
valid?}

To study the validity of the outputs of the fault localiser, 
we study the number of errors for the predicted robust and 
non-robust words. 
We do this by generating speech containing the 
predicted robust and non-robust words for each ASR tested. 
%Specifically, we use the 
%explanations of the \SMLT framework for the noise transformation for the 
%accents dataset. 
%\revise{
We choose an $\omega$ of three, three and two for GCP, MS Azure and IBM
respectively to choose the non-robust words ({\em see 
\Cref{alg:fault-loc}}). We choose the robust 
words from the set of words that do not show any errors in the presence
of noise ($\mathit{count\_diff}$ = 0 in {\em 
\Cref{alg:fault-loc}}) for these specific ASR systems.
%}
Specifically, we test whether the robust and 
non-robust words identified by the fault localiser in the 
Accents dataset are robust in the presence of noise.
Our goal is to show that if noise is added to speech 
containing these non-robust words, the ASR will be less likely to recognise 
them. Vice-versa, if noise is added to the predicted robust-words they are 
less likely to be affected. 

To generate the speech from the output we generate sentences containing
the robust and non-robust words predicted by the fault localiser 
for each ASR using a grammar and then 
use a text-to-speech (TTS) service to generate speech. The actual randomly 
selected robust and non-robust words (in bold) and the examples
of the sentences generated by the grammar can be seen in 
\Cref{tab:gram-sentences}. The grammars themselves can be seen in 
\Cref{fig:rq3-grammars}.
%\revise{
We use the Google TTS for MS Azure and we use the 
Microsoft Azure TTS for GCP and IBM to generate the speech.
%} \
%\todo{verify the previous sentence with Sai}

To evaluate the generality of outputs of the fault 
localisation technique, we use the speech produced by the TTS  
and then add noise to that speech. This speech is used to generate a 
transcript from the ASR and the transcript is used to evaluate how 
many of the predicted robust and non-robust words are incorrect in the 
transcript. We add the most noise possible to the TTS speech in our \SMLT 
framework. Specifically, the signal to noise (SNR) ratio is 2. We use 
the TTS generated speech for 50 sentences for each of the robust and 
non-robust cases. Each sentence has either a robust or a non-robust 
word.

The results of the experiments are seen in \Cref{tab:explanation-generality}.
In the transcript of the speech with noise added at SNR 2, robust words 
show {\em zero} error for the predicted robust words for Microsoft and 
Google Cloud and 21 errors for IBM. The non-robust words
on the other hand had 23, 15 and 30 errors. Thus, the predicted
non-robust words have a higher propensity for errors than the 
robust words. 

\begin{result}
	The outputs of the fault localisation techniques are general and valid.  
\end{result}

\begin{table}
%	
	\begin{minipage}[t]{0.4\textwidth}
	\caption{Transcript Errors}
	\centering
	{\scriptsize
    \begin{tabular}{lrrrr}
        \toprule
        \multicolumn{2}{l}{ASR}  & \makecell{Transcript\\Errors} \\ \midrule
        \multicolumn{2}{l}{Microsoft (MS)} & \\
        & \textit{Robust} & 0 \\ 
        & \textit{Non-Robust} & 23  \\ 
        \cmidrule{1-3}
        \multicolumn{2}{l}{Google Cloud (GCP)} & \\
         & \textit{Robust} & 0\\ 
        & \textit{Non-Robust} & 15\\ 
        \cmidrule{1-3}
        \multicolumn{2}{l}{IBM Watson (IBM)} & \\
        & \textit{Robust} & 21  \\ 
        & \textit{Non-Robust} & 30 \\ 
        \bottomrule
    \end{tabular}}
    \label{tab:explanation-generality}
	\end{minipage}
%	
	\centering
	\begin{minipage}[t]{0.55\textwidth}
	\caption{Grammarly Scores}
	\centering
	{\scriptsize
	\centering
    \begin{tabular}{lrrrr}
        \toprule
        \multicolumn{2}{l}{ASR}  & \makecell{Overall\\Score} & 
        \makecell{Correctness} & \makecell{Clarity} \\ \midrule
        \multicolumn{2}{l}{Microsoft (MS)} & \\
        & \textit{Robust} & 99 & \multirow{8}{*}{\makecell{Looking\\Good}} &  
        \multirow{8}{*}{\makecell{Very\\Clear}}\\ 
        & \textit{Non-Robust} & 99 & &  \\ 
        \cmidrule{1-3}
        \multicolumn{2}{l}{Google Cloud (GCP)} & \\
         & \textit{Robust} & 100 &  & \\ 
        & \textit{Non-Robust} & 99 & & \\ 
        \cmidrule{1-3}
        \multicolumn{2}{l}{IBM Watson (IBM)} & \\
        & \textit{Robust} & 100 & &  \\ 
        & \textit{Non-Robust} & 96 & & \\ 
        \bottomrule
    \end{tabular}}
    \label{tab:gram-eval}
	\end{minipage}
\end{table}

\smallskip \noindent
\textbf{Note on grammar validity:}
Since the grammars used by us to validate the explanations of 
\SMLT are handcrafted, they may be prone to errors. To verify these 
hand crafted grammars, we use 100 sentences produced by each grammar 
and use the online tool Grammarly~\cite{grammarly} to investigate the 
semantic and syntactic correctness of the sentences and the clarity. 
The sentences generated by the grammars have a high overall average 
score of 98.33 out of 100, with the lowest being 96 
(\textit{see \Cref{tab:gram-eval}}). On the correctness and clarity 
measure, all the sentences generated by the grammars score 
{\em Looking Good} and {\em Very Clear}. 
%
%\begin{figure}[t]
%\begin{center}
%\includegraphics[scale=0.25]{figs/Explanability-Generality.png}
%\end{center}
%\caption{Incorrect robust and non-robust transcript errors}
%\label{fig:explanation-generality}
%%\vspace{-0.2in}
%\end{figure}

%\begin{table}
%\centering
%	\resizebox{\linewidth}{!}{
%    \begin{tabular}{lrrrr}
%        \toprule
%        \multicolumn{2}{l}{ASR}  & \makecell{Transcript\\Errors} \\ \midrule
%        \multicolumn{2}{l}{Microsoft (MS)} & \\
%        & \textit{Robust} & 0 \\ 
%        & \textit{Non-Robust} & 23  \\ 
%        \cmidrule{1-3}
%        \multicolumn{2}{l}{Google Cloud (GCP)} & \\
%         & \textit{Robust} & 0\\ 
%        & \textit{Non-Robust} & 15\\ 
%        \cmidrule{1-3}
%        \multicolumn{2}{l}{IBM Watson (IBM)} & \\
%        & \textit{Robust} & 21  \\ 
%        & \textit{Non-Robust} & 30 \\ 
%        \bottomrule
%    \end{tabular}}
%    \label{tab:gram-eval}
%	\caption{Transcript Errors}
%\end{table}


\smallskip \noindent
\textbf{RQ4: Can the fault localiser be used to 
highlight unfairness?}


\begin{table*}[t]
\caption{Average words mispredictions in the Accents dataset using the \SMLT localisation techniques}
\centering
	{ \scriptsize
    \begin{tabular}{lr rrrrrrr rrr rr}
        \toprule
        \multicolumn{1}{l}{}  & \multicolumn{7}{c} {Accents} \\ \cmidrule(lr){2-8}
%         & \multicolumn{2}{c} {RAVDESS} & \multicolumn{2}{c} {\makecell{Nigerian/Midlands\\English}}  \cmidrule(lr){9-10} \cmidrule(lr){11-12}
        \multicolumn{1}{l}{}  & English & Ganda & French & Gujarati & 
        Indonesian &	Korean & 	Russian 
%        &  Male & Female & Midlands & Nigerian 
        \\ \midrule
        
        \textbf{\makecell{ASR Sensitivity}} \\
        \multicolumn{1}{r}{\textit{GCP}} & 1.21 & 1.51 & 1.21 & 1.17 & 1.07 & 1.55 & 1.64\\
        \multicolumn{1}{r}{\textit{IBM}} & 1.03 & 1.94 & 1.38 & 1.35 & 1.48 & 1.92 & 1.70 \\
        \multicolumn{1}{r}{\textit{MS Azure}} & 0.47 & 0.66 & 0.40 & 0.48 & 0.36 & 0.87 & 0.63 \\
        \textbf{\makecell{Transition Sensitivity}} \\
        
        \multicolumn{1}{r}{\textit{Clipping}} & 2.00 & 2.53 & 2.12 & 2.60 & 2.29 & 2.81 & 3.13 \\
		\multicolumn{1}{r}{\textit{Drop}} & 0.30 & 1.02 & 0.52 & 0.54 & 0.57 & 1.15 & 0.74 \\
		\multicolumn{1}{r}{\textit{Frame}} & 0.38 & 0.89 & 0.68 & 0.56 & 0.51 & 1.19 & 0.65 \\
		\multicolumn{1}{r}{\textit{Noise}} & 0.57 & 1.60 & 0.85 & 1.27 & 0.71 & 1.74 & 1.54 \\
		\multicolumn{1}{r}{\textit{LP}} & 1.72 & 2.22 & 1.90 & 1.79 & 1.58 & 1.98 & 2.13 \\
		\multicolumn{1}{r}{\textit{Amplitude}} & 0.17 & 0.15 & 0.11 & 0.12 & 0.06 & 0.20 & 0.16 \\
		\multicolumn{1}{r}{\textit{HP}} & 0.74 & 0.75 & 0.38 & 0.22 & 0.49 & 0.64 & 0.76 \\
		\multicolumn{1}{r}{\textit{Scale}} & 1.38 & 1.79 & 1.42 & 0.90 & 1.54 & 1.89 & 1.45 \\
        
        \bottomrule
    \end{tabular}}
    \label{tab:localiser-accents-errors}
\end{table*}


The goal of this RQ is to investigate if the output of \Cref{alg:fault-loc}
can call attention to bias between different groups. Specifically, we 
evaluate if some groups show fewer faults, on average than others. 
To this end, we use the fault localisation algorithm 
(\textit{\Cref{alg:fault-loc}}) on the accents dataset and 
record the number of words incorrect in the transcript, on average for
each group of the accents dataset. This is done for each ASR under test. 
%and for each transformation. \revise{
It is also important to note that 
this technique uses no ground truth data and requires no manual input. 
This technique is designed to work with just the speech data and metadata
(groups).
%}

\Cref{tab:localiser-accents-errors} shows the average word drops across 
all transformations for the accents dataset for each ASR under test. 
Speech from native-English speakers shows the lowest average word drops for
the IBM Watson ASR and the third lowest for GCP and MS Azure ASRs.
%On average, speech from non native-English speakers generates 
%57.9\%, 11.9\% and 20.03\% more word drops than speech from native-English
%speakers for IBM Watson, GCP and MS Azure respectively. 
%
We also investigate the average word drops for each transformation 
in \SMLT averaged across all ASRs. 
Speech from native English speakers has the lowest average word drops for the 
Clipping, two types of frame drops and noise transformations and the second 
lowest errors for the low-pass filter transformation. 
(\textit{see \Cref{tab:localiser-accents-errors}}). 
%Speech from non-native 
%English speakers has 28.9\%, 154.4\%, 96.03\%, 125.7\% and 12.3\% more 
%average word drops than speech from native English speakers for the
%clipping, drop, frame, noise and low-pass filter transformations 
%respectively. 
%
For the rest of the transformations, namely amplitude, high-pass filter and 
scaling, we find that both speech from non-native English speakers and speech from native 
English speakers have comparable average word drops (\textit{see 
\Cref{tab:localiser-accents-errors}}). 
%Speech from non-native 
%English speakers generates less average word drops in amplitude (21.4\%) and 
%high-pass filters (27.18\%) and only slightly more (8.88\%) in comparison
%to native English speakers. 
%\revise{
This result is consistent with results
seen in RQ1.
%} 
%\todo{results seem too consistent? Investigate for bug.}

\begin{result}
The technique seen in \Cref{alg:fault-loc} can be used to highlight bias 
in speech and the results are consistent with RQ1.	
\end{result}



%\begin{figure*}[t]
%\begin{center}
%\resizebox{\linewidth}{!}{
%\begin{tabular}{cccc}
%\includegraphics[scale=0.15]{figs/Accents-Localiser-ASR-1-Errors.png} &
%\includegraphics[scale=0.15]{figs/Accents-Localiser-Transition-1-Errors.png} &
%\includegraphics[scale=0.15]{figs/Accents-Localiser-Transition-2-Errors.png} & 
%\includegraphics[scale=0.15]{figs/Accents-Localiser-Transition-3-Errors.png}\\
%\\
%{\bf (a)} & {\bf (b)} & {\bf (c)} & {\bf (d)} \\
%\end{tabular}}
%
%\end{center}
%\caption{Sensitivity analysis for the Accents dataset using the \SMLT localisation techniques}
%\label{fig:localiser-accents-errors}
%\end{figure*}




%\subsection{RQ5: When should \SMLT not be used?}
%In this research question, we aim to uncover cases where \SMLT should not be 
%used to uncover fairness violations. 
%%We try to identify conditions where identifying 
%%bias through robustness using our \SMLT technique leads to misrepresentation.
%Specifically, we attempt to identify conditions where using our \SMLT technique 
%may lead to misrepresentation of bias.
%
%%\revise{
%Intuitively, the identification of fairness errors involves checking 
%how robustly ASR systems behave when the input speech is subject to a 
%metamorphic transformation. If the accuracy of the ASR system is poor for the 
%original speech (i.e. w/o any metamorphic transformation), then there is little 
%room for the accuracy to become worse. In such cases, the designer should focus 
%on improving the quality of the ASR prediction before examining the robustness 
%of these predictions. In the following, we discuss two scenarios to concretely 
%highlight the usage scenario of \SMLT. 
%%}
%
%%robustness has meaning only when there is room for 
%%the speech to degrade. In cases where further degradation is not possible 
%%robustness is meaningless because the speech is {\em robustly bad}. 
%%One must focus on improving the quality of the ASR prediction before 
%%examining the robustness of these predictions.
%
%%Firstly, consider the scenario shown in \Cref{fig:avg-word-lev-dist}. 
%
%%\revise{
%We capture the average word-level Levenshtein distances 
%($d_k$ in \Cref{alg:test-gen}) found in the various datasets used. 
%Firstly, we consider the case for African American Vernacular 
%English~\cite{aave} (AAVE) dataset. We find results in line with a recent 
%work~\cite{racialASR} which finds racial disparities between white 
%and black speakers in ASR systems. In our work, we find that 
%AAVE dataset exhibits significantly higher word-level Levenshtein distance 
%than speech from the Midlands in the UK~\cite{uk-midlands-dataset}
%(\textit{see \Cref{tab:avg-word-lev-dist}}). It is also interesting
%to note that we do not use any ground truth data to reach this conclusion. 
%%In addition, we find minor disparities between groups such as 
%%the accented
%%english speech of the various native English speakers
%%(\textit{see \Cref{fig:avg-word-lev-dist} (b)}), 
%%males and females~\cite{ravdess} 
%%(\textit{see \Cref{fig:avg-word-lev-dist} (c)}) and the accented
%%speech of Nigerian English and UK Midlands English
%%(\textit{see \Cref{fig:avg-word-lev-dist} (d)}).
%%\revise {
%Secondly, we consider cases where we find minor disparities between other groups.
%In particular, disparities between the accented speech of speakers from the 
%Accent dataset~\cite{accents} (\textit{see \Cref{tab:avg-word-lev-dist}}), 
%speech from males and females~\cite{ravdess} 
%(\textit{see \Cref{tab:avg-word-lev-dist}}) and the accented
%speech of Nigerian English speakers and UK Midlands English 
%speakers~\cite{nigerian-english,uk-midlands-dataset} 
%(\textit{see \Cref{tab:avg-word-lev-dist}}) are observed to be minor.
%%}. 
%%}
%
%%\revise{
%Out of the two scenarios, as explored in the preceding paragraph, we envision 
%that \SMLT should be used for the latter case i.e. when the disparity in word 
%error rates is minor between the concerned groups. In other words, the original 
%speech from the different groups exhibit similar error rates in the ASR system. 
%%Specifically, to highlight bias between speech from groups that on the surface seem to
%%perform equally well. 
%\revise{As a concrete example, consider the behaviour when the two datasets considered are AAVE and UK Midlands. 
%Our \SMLT technique shows that speech from AAVE speakers has less errors than the speech from the Midlands UK speakers (\textit{see \Cref{fig:aave-uk-midlands-errors}} in the Appendix).}
%However, this is because of the significantly higher error rates in the 
%original speech from the AAVE datasets than speech from the Midlands in the 
%UK~\cite{uk-midlands-dataset} (\textit{see \Cref{tab:avg-word-lev-dist}}). This 
%example shows a scenario when the results from \SMLT can capture the misrepresentation of 
%bias. Therefore, we suggest that our \SMLT technique should be used for comparing 
%speech from groups that otherwise exhibit similar performance.
%%}
%
%%This robustness is meaningless because the speech is just 
%%{\em robustly bad}. Our \SMLT technique is suitable when comparing
%%speech from groups that otherwise exhibit similar performance.
%
%\begin{result}
%	\SMLT should not be used in cases where there is obvious disparity in 
%	the performance of the ASR between groups. The groups should have similar 
%	differential error rates for a pair of ASR systems under test.
%\end{result}

%\begin{figure*}[t]
%\begin{center}
%\resizebox{\linewidth}{!}{
%\begin{tabular}{cccc}
%\includegraphics[scale=0.15]{figs/AAVE_UK-Total-Diff-Lev.png} &
%\includegraphics[scale=0.15]{figs/Accents-Total-Diff-Lev.png} &
%\includegraphics[scale=0.15]{figs/RAVDESS-Total-Diff-Lev.png} &
%\includegraphics[scale=0.15]{figs/Nigeria_UK_Midlands-Total-Diff-Lev.png}  \\
%\\
%{\bf (a)} & {\bf (b)} & {\bf (c)} & {\bf (d)}  \\
%\end{tabular}}
%
%\end{center}
%\caption{Average word-level Levenshtein distance}
%\label{fig:avg-word-lev-dist}
%\end{figure*}

%\begin{table*}[t]
%\caption{Average word-level Levenshtein distance}
%\centering
%	{\resizebox{\linewidth}{!}{
%    \begin{tabular}{lr rrrrrrr rrr rr r}
%        \toprule
%        \multicolumn{1}{l}{}  & \multicolumn{7}{c} {Accents} & \multicolumn{2}{c} {RAVDESS} & \multicolumn{2}{c} {\makecell{Nigerian/Midlands\\English}} & \multirow{3}{*}{AAVE} \\ \cmidrule(lr){2-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12}
%        \multicolumn{1}{l}{}  & English & Ganda & French & Gujarati & 
%        Indonesian &	Korean & 	Russian &  Male & Female & Midlands & Nigerian\\ \midrule
%        \textbf{\makecell{ASR Sensitivity}} \\
%		\multicolumn{1}{r}{\textit{MS IBM}} & 0.09 & 0.15 & 0.08 & 0.15 & 0.15 & 0.30 & 0.18 & 0.00 & 0.02 & 0.16 & 0.26 & 0.65 \\
%		\multicolumn{1}{r}{\textit{GCP IBM}}& 0.11 & 0.21 & 0.11 & 0.15 & 0.16 & 0.35 & 0.18 & 0.00 & 0.03 & 0.18 & 0.27 & 0.70  \\
%		\multicolumn{1}{r}{\textit{MS GCP}} & 0.13 & 0.23 & 0.12 & 0.15 & 0.14 & 0.38 & 0.22 & 0.00 & 0.04 & 0.09 & 0.24 & 0.51 \\
%
%        \bottomrule
%    \end{tabular}}}
%    \label{tab:avg-word-lev-dist}
%\end{table*}


%\begin{figure}[h]
%\begin{center}
%\includegraphics[scale=0.35]{figs/AAVE_UK-Total-Errors.png}
%\end{center}
%\caption{\revise{Errors for the AAVE/UK Midlands dataset}}
%\label{fig:aave-uk-midlands-errors}
%%\vspace{-0.2in}
%\end{figure}






==> FASE 2021/threats.tex <==
\section{Threats to Validity}
\label{sec:threats}

\smallskip \noindent
\textbf{User Study:} In conducting the study, two assumptions were made. 
Firstly, we assume that the degree to which comprehensibility changes when 
subject to transformations is independent of the characteristics of the 
speaker’s voice. Secondly, we assume that the speech is reflective of the 
broader English language. 
%That is we assume that the comprehensibility of 
%speech when subject to transformations is independent of the words 
%contained in it. 
In future work a larger scale user study could 
be performed to verify the results.

\smallskip \noindent
\textbf{ASR Baseline Accuracy:} 
%\revise{
\SMLT measures the degradation of the speech to characterise
the unfairness amongst groups and ASR systems. If the baseline error rate 
is very high, then the room for further degradation is very low. 
\revise{As a result, \SMLT expects 
ASR services to have a high baseline accuracy. To mitigate this threat, we
use state-of-the-art commercial ASR systems which have high baseline accuracies.}

\smallskip \noindent
\textbf{Completeness and Speech Data:}
%\revise{ 
\SMLT is incomplete, by design, in the discovery 
of fairness violations. \SMLT is limited by the speech data and the groups
of this speech data used to test these ASR systems. With new data and 
new groups, it is possible to discover more fairness violations. 
The practitioners need to provide data to discover these. In our 
view, this is a valid assumption because the developers of these 
systems have a large (and growing) corpus of such speech data. It is 
also important to note that \SMLT does not need the ground truth 
transcripts for this speech data and such speech data is easier to obtain. 
%}

\smallskip \noindent
\textbf{Fault Localisation:}
%\revise{ 
To test \SMLT's fault localisation, we identify the robust and non-robust 
words in the speech and subsequently construct sentences (with the aid 
of a grammar). These sentences are then converted to speech using
a text-to-speech (TTS) software and the performance of the robust and non-
robust words is measured. In the future, we would like to repeat the same 
experiment with a fixed set of speakers, which allows us capture the 
peculiarities of speech in contrast to the usage of TTS software.
%}

%\smallskip \noindent
%\textbf{Destructive Transformations:} 
%It is possible that the metamorphic transformations we use to generate 
%degradations also make the speech incomprehensible. To alleviate this 
%threat, we perform a user study with 200 users leveraging Amazon's 
%mTurk platform and verify that the comprehensibility of the 
%speech is not too adversely affected. 


%To alleviate this, we investigate the
%phenomenon and propose guidelines to practitioners for fairness
%testing ({\em see RQ5}).
%}


%\todo{Sakshi write threats}

==> Methodology-UserStudy.tex <==
\smallskip \noindent
\textbf{User Study:}
\label{sec:user-study-process}
In the course of our study, we subject speech signals to various metamorphic transformations (as explained in the preceding section) to test the overall robustness of ASR systems to these transformations. However, considering the full range of metamorphic transformations \revise{may} not useful since certain transformations deform speech to such an extent that it \revise{may not} be recognised any longer. In order to identify the set of transformations that are meaningful to consider, we conducted a study on relative comprehensibility of the transformed speech. The user study sought to determine whether the metamorphic transformations applied to the speech resulted in a speech that was still comprehensible to humans. Specifically, we seek to identify the degree to which the speech remains comprehensible as the intensity of each transformation is increased.


\textbf{User Study Setup:} We conducted a user study using Amazon’s mTurk platform. In particular, 200 participants were presented with an audio file containing speech utterances by a {\em female native English speaker}. In addition, the audio clip contained nearly all the sounds in the English language to represent the full spectrum of the language, as found in Speech Accent Archive~\cite{accents}. Users were presented with the original audio file along with a set of transformed speech files in order of increasing intensity. For instance, in the case of the "Scale" transformation, participants were first presented with a file that was slightly slowed down and subsequent files were slowed down even further. Users then rated the comprehensibility of the speech files in comparison to the original audio file. The rating was on a 1 to 10 scale, where "10" refers to the case where the modified speech file was just as comprehensible as the original speech and "1" refers to the case where 
the modified speech was not comprehensible at all.  

Participants were required to rate the comprehensibility of the entire set of transformations under 
study i.e. Amplitude, Clipping, Drop, Frame, Highpass, Lowpass, Noise and Scale 
(see~\Cref{fig:soundwave-transform}). The average score of each transformation was used to determine 
the comprehensibility score. In general, we see that 
the comprehensibility of the speech tends to go down as the intensity of the transformation increases, 
as observed in~\Cref{fig:user-study-results}. We present a comprehensive analysis of the user study results in {\bf RQ2}. 

%\smallskip \noindent
%\textbf{Caveats:} In conducting the study, two assumptions were made. Firstly, we assume that the degree to which comprehensibility changes when subject to transformations is independent of the characteristics of the speaker’s voice. Secondly, we assume that the speech is reflective of the broader English language. That is we assume that the comprehensibility of speech when subject to transformations is independent of the words contained in it. In the fullness of time, a larger scale user study could be performed to verify the results.

%\todo{Check: Caveats section is possibly superfluous. Possibly moved to threats to validity.}


==> motivation.tex <==
\section{Motivation}

\todo{Fairness in ASR}

%BLAH


